Instance-Level Composed Image Retrieval

The progress of composed image retrieval (CIR), a popular research direction in image retrieval, where a combined visual and textual query is used, is held back by the absence of high-quality training and evaluation data. We introduce a new evaluation dataset, i-CIR, which, unlike existing datasets, focuses on an instance-level class definition. The goal is to retrieve images that contain the same particular object as the visual query, presented under a variety of modifications defined by textual queries. Its design and curation process keep the dataset compact to facilitate future research, while maintaining its challenge-comparable to retrieval among more than 40M random distractors-through a semi-automated selection of hard negatives. To overcome the challenge of obtaining clean, diverse, and suitable training data, we leverage pre-trained vision-and-language models (VLMs) in a training-free approach called BASIC. The method separately estimates query-image-to-image and query-text-to-image similarities, performing late fusion to upweight images that satisfy both queries, while down-weighting those that exhibit high similarity with only one of the two. Each individual similarity is further improved by a set of components that are simple and intuitive. BASIC sets a new state of the art on i-CIR but also on existing CIR datasets that follow a semantic-level class definition. Project page: https://vrg.fel.cvut.cz/icir/.

==> fig/fig_illustration_dataset_extended.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{fig/i_cir.pdf}
    \caption{\emph{Illustration of \dataset}. Each instance consists of a set of query images and query texts, which are combined to form composed queries simulating realistic retrieval intents. For each composed query, the database includes composed positives that depict the same instance as the query image, modified according to the query text. Additionally, the database contains three categories of hard negatives: visual hard negatives (same or similar instance, different text), textual hard negatives (different instance, fully or matching text), and composed hard negatives (misleading combinations of both).}
    \label{fig:dataset}
\end{figure}

==> fig/full_fig_performance_per_category.tex <==
\begin{figure*}[t]
    \centering
    \scalebox{1.}{
       \input{fig/fig_performance_per_visual_category}
    }
    \vspace{-5pt}
    \caption{\emph{Performance comparison per primary visual category.} mAP (\%) averaged over instance in the same primary-level category size, sorted by. Comparison between...
    \label{fig:performance_barplot_visual}
    \vspace{-5pt}
    }
\end{figure*}

\begin{figure*}[t]
    \centering
    \scalebox{1.}{
       \input{fig/fig_performance_per_textual_category}
    }
    \vspace{-5pt}
    \caption{\emph{Performance comparison per textual category.} mAP averaged over instance in the same primary-level category size, sorted by. Comparison between...
    \label{fig:performance_barplot_textual}
    \vspace{-5pt}
    }
\end{figure*}

==> tab/exp_results_general_cir.tex <==
\centering
\fontsize{7}{5}\selectfont
\setlength{\tabcolsep}{12pt}
\begin{tabular}{lccc}
\toprule
Method & \Th{fashion-iq} & \Th{cirr} & \Th{circo} \\ \midrule
Text & 9.33 & 26.66 & 4.10 \\
Image & 1.43 & 11.73 & 2.61 \\
Text + Image & 3.93 & 19.02 & 5.61 \\
Text $\times$ Image & 10.67 & 29.37 & 11.12 \\
\midrule
\picword & 10.52 & \ts{29.75} & 8.16 \\
\searle & \ts{10.70} & \tb{31.50} & \ts{14.48} \\ 
\weicom & 6.77 & 18.84 & 10.61 \\ 
\cirevl & \tb{11.28} & 29.17 & \tb{19.67} \\ 
\freedom & 9.67 & 28.96 & 13.06 \\ \midrule
\ours & 9.04 & 24.38 & 14.47 \\
\ours$^\star$ & 10.54 & 26.83 & 13.94 \\
\bottomrule
\end{tabular}

==> tab/exp_results_imagenetr_recall.tex <==
\scriptsize
\begin{tabular}{lcccccccccc} \toprule
\multirow{2}{*}{\Th{Method}} & \multicolumn{2}{c}{\Th{Cartoon}} & \multicolumn{2}{c}{\Th{Origami}} & \multicolumn{2}{c}{\Th{Toy}} & \multicolumn{2}{c}{\Th{Sculpture}} & \multicolumn{2}{c}{\Th{Avg}} \\ \cmidrule{2-11}
& \Th{R@10}  & \Th{R@50}  & \Th{R@10}  & \Th{R@50}  & \Th{R@10}  & \Th{R@50}  & \Th{R@10}  & \Th{R@50}  & \Th{R@10}  & \Th{R@50}  \\ \midrule
Text    & 0.18 & 0.92 & 0.79 & 3.47 & 0.34 &  1.9 & 0.69 & 1.84 & 0.50 & 2.03 \\
Image  & 0.34 & 5.29 & 0.30 & 2.08 & 0.35 & 4.71 & 0.59 & 6.22 & 0.40 & 4.58 \\
Text + Image     2.27 & 15.13 & 2.49 & 11.67 & 2.20 & 13.83 & 1.75 & 12.51 & 2.18 & 13.28\\  
Text $\times$ Image   & 8.90      & 19.45       & 11.32     & 23.31        & 7.97  &    18.22 &   9.10 & 19.16 & 9.32 & 20.04 \\
\midrule
\picword                       & 8.00       & 21.90      & 13.50      & 25.60      & 8.70        & 21.60 &       10.00 &       23.80 & 10.05 & 23.23 \\
\picword  (CC-3M)              & 7.35       & 18.53      & 12.79      & 25.54      & 10.39       & 22.96 &       10.24 &       23.76 & 10.19 & 22.70 \\
\picword  (LAION 2B-en)        & 8.17       & 20.86      & 14.08      & 25.06      & 8.73        & 22.07 &       10.43 &       23.63 & 10.35 & 22.91 \\
ARTEMIS w/ CompoDiff dataset   & 11.42      & 23.81      & 15.49      & 25.44      & 11.21       & 24.01 &       10.84 &       21.07 & 12.24 & 23.58 \\
CLIP4Cir w/ CompoDiff dataset  & 10.90      & 24.12      & 16.08      & 25.60      & 11.01       & 23.57 &       10.45 &       21.86 & 12.11 & 23.79 \\
\compodiff (T5-XL)             & 8.43       & 20.40      & 15.73      & 25.69      & 11.19       & 22.48 &       9.19  &       18.45 & 11.14 & 21.76 \\
\compodiff (CLIP+T5-XL)        & 12.91      & 24.40      & 17.22      & 26.40      & 11.57       & 26.11 &       11.53 &       22.54 & 13.31 & 24.86 \\
\compodiff (CLIP)              & 13.21      & 24.06      & 17.03      & 26.17      & 11.22       & 26.25 &       11.24 &       22.96 & 13.18 & 24.86 \\  
KEDs                           & 14.80      & 34.20      & \ts{23.50} & 34.80      & 16.50       & 36.30 &       17.40 &       36.40 & 18.00 & 35.40 \\
\midrule
\searle                & 10.17      & 30.32      & 17.02      & 32.00      & 8.23        & 9.10       & 11.60 &       32.41 & 11.76 & 30.96 \\
\weicom                        & 11.61      & 24.36      & 15.24      & 23.72      & 8.00        & 17.89      & 13.81 &         26.18 & 12.17 & 23.04 \\
\cirevl                        & \ts{19.20} & \ts{42.80} & 22.20      & \tb{43.10}  & \tb{30.20}  & \ts{41.30} & \ts{23.40} &  \ts{45.00 }& \ts{23.75} & \ts{43.05} \\

\freedom                          & \tb{23.77} & \tb{48.80} & \tb{32.86} & \ts{42.82} & \ts{25.71} & \tb{47.47} & \tb{27.87} & \tb{48.96} & \tb{27.55} & \tb{47.01} \\
\midrule
\rowcolor{LightSteelBlue1}
\ours   & 22.37 & 48.40 & 27.19 & 39.41 & 26.64 & 46.42 & 25.52 & 46.07 & 25.43 & 45.08 \\ 
\bottomrule
\end{tabular}


==> tex/abbrev.tex <==
%%% TEMPLATE TRICKS
\newcommand{\mypartight}[1]{\noindent {\bf #1}}
\newcommand{\myparagraph}[1]{\vspace{3pt}\noindent\textbf{#1}\xspace}

\newcommand{\alert}[1]{{\color{red}{#1}}}
\newcommand{\rebuttal}[1]{{\color{blue}{#1}}}
\newcommand{\paperadd}[1]{{\color{blue}{#1}}}
\newcommand{\gray}[1]{{\color{gray}{#1}}}

% Figures macros 
\newcommand{\fig}[2][1]{\includegraphics[width=#1\linewidth]{fig/#2}}
\newcommand{\figh}[2][1]{\includegraphics[height=#1\linewidth]{fig/#2}}
\newcommand{\figa}[2][1]{\includegraphics[width=#1]{fig/#2}}
\newcommand{\figah}[2][1]{\includegraphics[height=#1]{fig/#2}}

% Figures macros 
\newcommand{\figsup}[2][1]{\includegraphics[width=#1\linewidth]{fig_supp/#2}}
\newcommand{\figsuph}[2][1]{\includegraphics[height=#1\linewidth]{fig_supp/#2}}
\newcommand{\figsupa}[2][1]{\includegraphics[width=#1]{fig_supp/#2}}
\newcommand{\figsupah}[2][1]{\includegraphics[height=#1]{fig_supp/#2}}
\newcommand{\figsupc}[2][1]{\includegraphics[width=#1\linewidth,cfbox=OliveGreen 1.5pt 1.5pt]{fig_supp/#2}}
\newcommand{\figsupw}[2][1]{\includegraphics[width=#1\linewidth,cfbox=BrickRed 1.5pt 1.5pt]{fig_supp/#2}}
\newcommand{\figsupq}[2][1]{\includegraphics[width=#1\linewidth,cfbox=OrangeFrame 1.5pt 1.5pt]{fig_supp/#2}}
\newcommand{\bfigsupc}[2][1]{\includegraphics[width=#1\linewidth,height=#1\linewidth,cfbox=OliveGreen 1.5pt 1.5pt]{fig_supp/#2}}
\newcommand{\bfigsupw}[2][1]{\includegraphics[width=#1\linewidth,height=#1\linewidth,cfbox=BrickRed 1.5pt 1.5pt]{fig_supp/#2}}
\newcommand{\bfigsupq}[2][1]{\includegraphics[width=#1\linewidth,height=#1\linewidth,cfbox=OrangeFrame 1.5pt 1.5pt]{fig_supp/#2}}

% Figures macros 
\newcommand{\figreb}[2][1]{\includegraphics[width=#1\linewidth]{fig_reb/#2}}
\newcommand{\figrebh}[2][1]{\includegraphics[height=#1\linewidth]{fig_reb/#2}}
\newcommand{\figreba}[2][1]{\includegraphics[width=#1]{fig_reb/#2}}
\newcommand{\figrebah}[2][1]{\includegraphics[height=#1]{fig_reb/#2}}
\newcommand{\figrebc}[2][1]{\includegraphics[width=#1\linewidth,cfbox=OliveGreen 1.0pt 1.0pt]{fig_reb/#2}}
\newcommand{\figrebw}[2][1]{\includegraphics[width=#1\linewidth,cfbox=BrickRed 1.0pt 1.0pt]{fig_reb/#2}}
\newcommand{\figrebq}[2][1]{\includegraphics[width=#1\linewidth,cfbox=OrangeFrame 1.0pt 1.0pt]{fig_reb/#2}}
\newcommand{\bfigrebc}[2][1]{\includegraphics[width=#1\linewidth,height=#1\linewidth,cfbox=OliveGreen 1.0pt 1.0pt]{fig_reb/#2}}
\newcommand{\bfigrebw}[2][1]{\includegraphics[width=#1\linewidth,height=#1\linewidth,cfbox=BrickRed 1.0pt 1.0pt]{fig_reb/#2}}
\newcommand{\bfigrebq}[2][1]{\includegraphics[width=#1\linewidth,height=#1\linewidth,cfbox=OrangeFrame 1.0pt 1.0pt]{fig_reb/#2}}
%--------------------------------------------------------------------------------
% Table rows/columns macros 
\newcommand{\mr}[2]{\multirow{#1}{*}{#2}}
\newcommand{\mc}[2]{\multicolumn{#1}{c}{#2}}
\newcommand{\Th}[1]{\textsc{#1}}
\newcommand{\tb}[1]{\textbf{#1}}

%--------------------------------------------------------------------------------
% stdev in tables
\newcommand{\stddev}[1]{\scriptsize{$\pm#1$}}

\newcommand{\diffup}[1]{{\color{OliveGreen}{($\uparrow$ #1)}}}
\newcommand{\diffdown}[1]{{\color{BrickRed}{($\downarrow$ #1)}}}

%--------------------------------------------------------------------------------
%algorithm

%--------------------------------------------------------------------
% spaces: useful for tabulars
\def\nmsp{\hspace{-6pt}}
\def\nssp{\hspace{-3pt}}
\def\nxssp{\hspace{-1pt}}
\def\zsp{\hspace{0pt}}
\def\xssp{\hspace{1pt}}
\def\ssp{\hspace{3pt}}
\def\msp{\hspace{6pt}}
\def\lsp{\hspace{12pt}}
\def\xlsp{\hspace{20pt}}
%--------------------------------------------------------------------

\newcommand{\head}[1]{{\smallskip\noindent\bf #1}}
\newcommand{\equ}[1]{(\ref{equ:#1})\xspace}
\newcommand{\eq}[1]{(\ref{eq:#1})\xspace}

%--------------------------------------------------------------------

\def\l1{\ensuremath{\ell_1}\xspace}
\def\l2{\ensuremath{\ell_2}\xspace}

%--------------------------------------------------------------------

\newcommand{\tran}{^\top}
\newcommand{\mtran}{^{-\top}}
\newcommand{\zcol}{\mathbf{0}}
\newcommand{\zrow}{\zcol\tran}

% \newcommand{\ind}{\mathbbm{1}}
\newcommand{\ind}{\mathds{1}}
\newcommand{\expect}{\mathbb{E}}
\newcommand{\nat}{\mathbb{N}}
\newcommand{\zahl}{\mathbb{Z}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\proj}{\mathbb{P}}
\newcommand{\prob}{\mathbf{Pr}}

\newcommand{\mif}{\textrm{if }}
\newcommand{\other}{\textrm{otherwise}}
\newcommand{\minimize}{\textrm{minimize }}
\newcommand{\maximize}{\textrm{maximize }}
% \newcommand{\st}{\textrm{subject to }}

\newcommand{\id}{\operatorname{id}}
\newcommand{\const}{\operatorname{const}}
\newcommand{\sgn}{\operatorname{sgn}}
\newcommand{\var}{\operatorname{Var}}
\newcommand{\mean}{\operatorname{mean}}
\newcommand{\trace}{\operatorname{tr}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\vect}{\operatorname{vec}}
\newcommand{\cov}{\operatorname{cov}}

\newcommand{\softmax}{\operatorname{softmax}}
\newcommand{\clip}{\operatorname{clip}}

\newcommand{\defn}{\mathrel{:=}}
\newcommand{\peq}{\mathrel{+\!=}}
\newcommand{\meq}{\mathrel{-\!=}}

\newcommand{\floor}[1]{\left\lfloor{#1}\right\rfloor}
\newcommand{\ceil}[1]{\left\lceil{#1}\right\rceil}
\newcommand{\inner}[1]{\left\langle{#1}\right\rangle}
\newcommand{\norm}[1]{\left\|{#1}\right\|}
\newcommand{\frob}[1]{\norm{#1}_F}
\newcommand{\card}[1]{\left|{#1}\right|\xspace}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\der}[3][]{\frac{d^{#1}#2}{d#3^{#1}}}
\newcommand{\pder}[3][]{\frac{\partial^{#1}{#2}}{\partial{#3^{#1}}}}
\newcommand{\ipder}[3][]{\partial^{#1}{#2}/\partial{#3^{#1}}}
\newcommand{\dder}[3]{\frac{\partial^2{#1}}{\partial{#2}\partial{#3}}}

\newcommand{\wb}[1]{\overline{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\vA}{\mathbf{A}}
\newcommand{\vB}{\mathbf{B}}
\newcommand{\vC}{\mathbf{C}}
\newcommand{\vD}{\mathbf{D}}
\newcommand{\vE}{\mathbf{E}}
\newcommand{\vF}{\mathbf{F}}
\newcommand{\vG}{\mathbf{G}}
\newcommand{\vH}{\mathbf{H}}
\newcommand{\vI}{\mathbf{I}}
\newcommand{\vJ}{\mathbf{J}}
\newcommand{\vK}{\mathbf{K}}
\newcommand{\vL}{\mathbf{L}}
\newcommand{\vM}{\mathbf{M}}
\newcommand{\vN}{\mathbf{N}}
\newcommand{\vO}{\mathbf{O}}
\newcommand{\vP}{\mathbf{P}}
\newcommand{\vQ}{\mathbf{Q}}
\newcommand{\vR}{\mathbf{R}}
\newcommand{\vS}{\mathbf{S}}
\newcommand{\vT}{\mathbf{T}}
\newcommand{\vU}{\mathbf{U}}
\newcommand{\vV}{\mathbf{V}}
\newcommand{\vW}{\mathbf{W}}
\newcommand{\vX}{\mathbf{X}}
\newcommand{\vY}{\mathbf{Y}}
\newcommand{\vZ}{\mathbf{Z}}

\newcommand{\va}{\mathbf{a}}
\newcommand{\vb}{\mathbf{b}}
\newcommand{\vc}{\mathbf{c}}
\newcommand{\vd}{\mathbf{d}}
\newcommand{\ve}{\mathbf{e}}
\newcommand{\vf}{\mathbf{f}}
\newcommand{\vg}{\mathbf{g}}
\newcommand{\vh}{\mathbf{h}}
\newcommand{\vi}{\mathbf{i}}
\newcommand{\vj}{\mathbf{j}}
\newcommand{\vk}{\mathbf{k}}
\newcommand{\vl}{\mathbf{l}}
\newcommand{\vm}{\mathbf{m}}
\newcommand{\vn}{\mathbf{n}}
\newcommand{\vo}{\mathbf{o}}
\newcommand{\vp}{\mathbf{p}}
\newcommand{\vq}{\mathbf{q}}
\newcommand{\vr}{\mathbf{r}}
\newcommand{\Vs}{\mathbf{s}}
\newcommand{\vt}{\mathbf{t}}
\newcommand{\vu}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vw}{\mathbf{w}}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\vz}{\mathbf{z}}

\newcommand{\vone}{\mathbf{1}}
\newcommand{\vzero}{\mathbf{0}}

\newcommand{\valpha}{{\boldsymbol{\alpha}}}
\newcommand{\vbeta}{{\boldsymbol{\beta}}}
\newcommand{\vgamma}{{\boldsymbol{\gamma}}}
\newcommand{\vdelta}{{\boldsymbol{\delta}}}
\newcommand{\vepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\vzeta}{{\boldsymbol{\zeta}}}
\newcommand{\veta}{{\boldsymbol{\eta}}}
\newcommand{\vtheta}{{\boldsymbol{\theta}}}
\newcommand{\viota}{{\boldsymbol{\iota}}}
\newcommand{\vkappa}{{\boldsymbol{\kappa}}}
\newcommand{\vlambda}{{\boldsymbol{\lambda}}}
\newcommand{\vmu}{{\boldsymbol{\mu}}}
\newcommand{\vnu}{{\boldsymbol{\nu}}}
\newcommand{\vxi}{{\boldsymbol{\xi}}}
\newcommand{\vomikron}{{\boldsymbol{\omikron}}}
\newcommand{\vpi}{{\boldsymbol{\pi}}}
\newcommand{\vrho}{{\boldsymbol{\rho}}}
\newcommand{\vsigma}{{\boldsymbol{\sigma}}}
\newcommand{\vtau}{{\boldsymbol{\tau}}}
\newcommand{\vupsilon}{{\boldsymbol{\upsilon}}}
\newcommand{\vphi}{{\boldsymbol{\phi}}}
\newcommand{\vchi}{{\boldsymbol{\chi}}}
\newcommand{\vpsi}{{\boldsymbol{\psi}}}
\newcommand{\vomega}{{\boldsymbol{\omega}}}

\newcommand{\rLambda}{\mathrm{\Lambda}}
\newcommand{\rSigma}{\mathrm{\Sigma}}

%--------------------------------------------------------------------
% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
%

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\vs{\emph{vs\onedot}}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

% \newcommand{\ie}{\textit{i.e.}\xspace}
% \newcommand{\vs}{\textit{vs.}\xspace}
% \newcommand{\eg}{\textit{e.g.}\xspace}
% \newcommand{\etc}{\textit{e.t.c.}\xspace}
% \newcommand{\etal}{\textit{et al.}\xspace}

\usepackage[table]{xcolor}
\newcommand{\alertrow}{\rowcolor{red!10}} % soft red background

==> tex/abstract.tex <==
%This work addresses the lack of data, both for evaluation and training, for \emph{composed image retrieval} (CIR), where a combined visual and textual query is used.

%\vspace{-12pt}
The progress of \emph{composed image retrieval} (CIR), a popular research direction in image retrieval, where a combined visual and textual query is used, is held back by the absence of high-quality training and evaluation data.
%
We introduce a new evaluation dataset, \dataset, which, unlike existing datasets, focuses on an instance-level class definition. The goal is to retrieve images that contain the same particular object as the visual query, presented under a variety of modifications defined by textual queries. Its design and curation process keep the dataset compact to facilitate future research, while maintaining its challenge—comparable to retrieval among more than 40M random distractors—through a semi-automated selection of hard negatives. %\alert{We show that \dataset is as challenging as using a database with 20 million randomly selected distractor images, yet contains on average only 3,700 in query-specific databases.}
%\alert{—comparable to retrieval among 20M random distractors—}
To overcome the challenge of obtaining clean, diverse, and suitable training data, we leverage pre-trained vision-and-language models (VLMs) in a training-free approach called \ours. The method separately estimates query-image-to-image and query-text-to-image similarities, performing late fusion to upweight images that satisfy both queries, while downweighting those that exhibit high similarity with only one of the two. Each individual similarity is further improved by a set of components that are simple and intuitive.
% \alert{Each individual similarity is further improved by exploiting the compatibility and interplay between the visual and textual modalities in VLMs.}
\ours sets a new state of the art on \dataset but also on existing CIR datasets that follow a semantic-level class definition. Project page: \url{https://vrg.fel.cvut.cz/icir/}.


% Composed Image Retrieval (CIR), the task of retrieving images using combined image and text queries, traditionally operates at a class-level granularity, as exemplified by existing benchmarks such as Fashion-IQ and CIRR. However, these datasets contain significant annotation ambiguities, redundancy in either modality, and fail to provide challenging negatives, thus limiting fair model evaluation and meaningful progress. In this work, we introduce Instance-Level Composed Image Retrieval (ILCIR) task, arguing that instance-level retrieval aligns more closely with real-world applications, such as personalized photo collections. We present the \dataset dataset, comprising 100 carefully selected unique instances across diverse categories, annotated to guarantee challenging negative examples at image-only, text-only, and composed-query levels. We propose a simple yet effective method that sets a new state-of-the-art on \dataset and surpasses current methods on several existing CIR benchmarks.
% The proposed approach operates in a VLM's embedding space and combines two query modalities using an “and” operator, implemented via the multiplication of similarity scores. It introduces a projection of the image query into a subspace that suppresses non-semantic factors such as background, style, and dataset-specific bias. This projection is derived from text embeddings computed over a predefined object-centric corpus, and can be further refined using a “negative” corpus that encodes distractor concepts to be explicitly filtered out. The method is complemented by lightweight, training-free operations that act as effective best practices within retrieval pipelines, resulting in a simple yet powerful framework for composite image-text retrieval. Dataset and code will be publicly available.

% %Composed Image Retrieval (CIR) enables querying with a reference image combined with a modifying textual description, aiming to retrieve target images that reflect both visual and semantic aspects. Existing benchmarks predominantly focus on class-level CIR, such as Fashion-IQ and CIRR, but suffer from significant drawbacks, including ambiguous annotations, redundancy in image or text queries, and inadequate evaluation due to noisy negative samples. Furthermore, class-level retrieval scenarios are less representative of everyday real-world use-cases, where queries typically target specific instances rather than broader categories.To address these challenges, we introduce Instance-Level Composed Image Retrieval (ILCIR), a novel CIR benchmark explicitly designed for real-world applications. ILCIR comprises 100 meticulously curated instances across diverse categories such as landmarks, scenes, and objects, with approximately 1K query images and 300K database images. Each instance is associated with multiple challenging negative examples, rigorously annotated to ensure semantic and structural precision. This structure guarantees hard negative samples at three distinct levels—image-only, text-only, and their composed combination—providing a robust and fair evaluation environment.In addition, we propose a straightforward yet highly effective retrieval method that establishes new state-of-the-art performance on the ILCIR dataset and consistently surpasses existing methods on current CIR benchmarks. Our comprehensive experiments underscore the importance and practicality of instance-level retrieval, demonstrating its superiority and applicability for realistic scenarios. The ILCIR dataset and accompanying code will be publicly available, facilitating further research in this promising direction.

==> tex/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction accurately summarize our key contributions: the creation of an instance-level composed image retrieval dataset (\dataset) with challenging hard negatives, the proposal of a training-free CIR method (\ours) that leverages existing VLMs, and the demonstration of state-of-the-art performance on \dataset and multiple benchmarks. All claims are supported by detailed methodology and experiments in Sections 3–5, as also in supplementray material.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: We explicitly acknowledge in Sec.~3 (footnote) that our logical‐AND assumption may break down when one modality dominates (e.g., pure style edits or highly entangled image–text pairs like CIRCO). We point readers to additional method and dataset limitations in the supplementary material.  
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper contains no formal theorems or theoretical results requiring proof; it is entirely empirical and algorithmic.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: We give exhaustive details of our dataset construction (including LAION search and retrieve, filtering and annotation protocols) and our method (all pre-processing steps, corpora generation, hyper-parameters $k,\lambda,\alpha$, normalization statistics), and we commit to releasing both the dataset and code with scripts to reproduce every result.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{}
    \item[] Justification: Both \dataset dataset and code will be made publicly available through our project page \url{https://vrg.fel.cvut.cz/icir/}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: The experimental section of both the main paper and supplementary material is exhaustive and detailed. It specifies all the details needed to understand the results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: Our method is training-free, so it does not involve sources of randomness such as weight initialization, optimization, or data shuffling.  
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Technical and implementation details are included in the supplementary material.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: We use only publicly available, license-annotated sources (\eg, LAION-derived URLs and rights-cleared repositories), and we respect licenses and site Terms of Service. All images in \dataset{} were reviewed by trained annotators; inappropriate, copyrighted, or privacy-sensitive content was removed. In categories where people are inherently present (\eg, apparel), we automatically pixelate faces and perform spot checks; no raw PII is released. \dataset{} is an evaluation-only benchmark, distributed under CC-BY-NC-SA with an explicit prohibition on surveillance/biometric or other privacy-invasive uses. We publish a misuse policy, provide a “Report misuse/PII” channel, honor takedown requests, and reserve the right to revoke access for violations. Our method is training-free and does not scrape private data, minimizing environmental and privacy risks. No human-subjects research was conducted (IRB not applicable). Overall, collection, curation, release, and documentation follow the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper explicitly discusses benefits and risks. On the positive side, instance-level composed retrieval can support cultural-heritage search (GLAM), assistive-vision use cases, product provenance, and reproducible evaluation of compositional models. On the negative side, we analyze dual-use pathways—including surveillance/profiling, indirect “object-of-interest” tracking (\eg, via distinctive belongings), fine-tuning our techniques on face/plate corpora, and misuse of crawl scripts—and we describe harms from both correct and incorrect system behavior. However, we exhaustively outline concrete mitigations too.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{}
    \item[] Justification: We release \dataset{} as an \emph{evaluation-only} benchmark under CC-BY-NC-SA with an explicit ban on surveillance/biometric and other privacy-invasive uses; access is governed by a misuse policy with revocation. Images are curated with a privacy-first process: annotators preferentially exclude PII, and in categories where people are intrinsic (\eg, apparel) we retain images but \emph{exhaustively pixelate} visible faces before release; we also filter watermarks, near-duplicates, and low-quality items, followed by manual spot checks. Any search/crawl scripts are released under the same restrictive license with hard-coded keyword blocks and documentation discouraging sensitive-content collection (IRB review recommended for modifications). The project page provides a prominent “Report misuse / PII” channel; we commit to prompt review, content takedown, and access revocation when warranted. We will periodically red-team object-level re-identification risks and update the release if failure modes are found. No identification models or person-level embeddings are released; our method is training-free and not tailored to biometric tasks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: We build on publicly available assets and cite them in the paper and project page. For data, we rely on LAION \emph{metadata} (CC-BY 4.0) and keep each image under its original source license. For models/code, we use public VLMs and toolchains under their original licenses and cite them: CLIP (MIT), OpenCLIP (Apache-2.0), and, for anonymization, InsightFace (MIT). Our own release is evaluation-only under CC-BY-NC-SA and does not alter upstream terms; LICENSE files and attributions are included in our repo.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}
    \item[] Justification: We release \dataset with a comprehensive datasheet detailing collection protocols, licensing, annotation guidelines, dataset statistics, and limitations; our code repository includes installation instructions, example scripts, configuration files for all experiments, and explicit CC-BY-NC-SA license information.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerYes{}
    \item[] Justification: We did not use crowdsourcing; all annotations were performed by salaried institutional staff. The supplemental material includes annotation guidelines/instructions. Annotators received domain and ethics training, and we ran weekly QA spot-checks and inter-annotator-agreement audits. Compensation exceeds the legal minimum (>\,80\% of a first-year PhD stipend with full social-security coverage). No participants were recruited, no demographic attributes were collected, and PII was removed/redacted; thus this work does not constitute human-subjects research, but we nevertheless followed our institution’s ethics policies throughout.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: This work does not constitute human-subjects research: no participants were recruited or interacted with; annotators were salaried staff performing routine labeling; no demographic or behavioral data were collected; and all images were sourced from public datasets with PII removed/pixelated prior to release. Under these conditions, IRB (or equivalent) review is not required per common definitions and institutional policies.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{}
    \item[] Justification: The core method development in this research does not involve LLMs.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> tex/conclusion.tex <==
\section{Conclusions}
\label{sec:concl}

%A new evaluation dataset for composed image retrieval at the instance level, \dataset, was introduced. It provides an important and long missing properly annotated dataset with explicitly incorporated hard negative examples of visual, textual, and composed nature. The dataset has the ambition of becoming an essential evaluation tool for CIR methods. Together with the dataset, a simple, efficient and flexible method, \ours, was proposed. The method compares favorably with all existing CIR methods in both categories: training-based and training-free. %The superior performance of \ours is demonstrated on \dataset, but also on a number of existing benchmarks, using standard evaluation protocols.

We introduced \dataset, an instance-level benchmark for composed image retrieval with \emph{explicit hard negatives} (visual, textual, and composed). It fills a long-standing gap by providing an ambiguity-free evaluation suite that rewards composition rather than single-modality shortcuts. We also presented \ours, a simple, efficient, \emph{training-free} method that compares favorably to both training-based and training-free baselines across benchmarks. \ours is built from a few transparent components, whose combination delivers strong accuracy, transfers well, and exhibits broad hyperparameter plateaus. We hope \dataset{} becomes a reliable target for assessing genuinely compositional retrieval, and that the simplicity of \ours catalyzes adoption and further advances.

%\paragraph{Acknowledgments.} This research was supported by (i) the Czech National Recovery Plan project CEDMO 2.0 NPO (MPO 60273/24/21300/21000) provided by the Ministry of Industry and Trade of the Czech Republic, (ii) the European Union's Horizon Europe programme under the Marie Sklodowska-Curie Postdoctoral Fellowship grant agreement No. 101205297, (iii) the European Union's Horizon Europe programme (grant agreement No. 101136568 - HERON - Hellenic Robotics Center of Excellence), (iv) the project ``Applied Research for Autonomous Robotic Systems” (MIS5200632), implemented within the framework of the National Recovery and Resilience Plan (NNRP) ``Greece 2.0” (Measure: 16618 - Basic and Applied Research) and funded by the European Union - NextGenerationEU, and (v) the CTU in Prague grant No. SGS23/173/OHK3/3T/13, and the CTU in Prague institutional support (Future fund). We acknowledge VSB – Technical University of Ostrava, IT4Innovations National Supercomputing Center, Czech Republic, for awarding this project (OPEN-33-67) access to the LUMI supercomputer, owned by the EuroHPC Joint Undertaking, hosted by CSC (Finland) and the LUMI consortium, through the Ministry of Education, Youth and Sports of the Czech Republic via the e-INFRA CZ project (ID: 90254). We acknowledge the access to the computational infrastructure of the OP VVV funded project CZ.02.1.01/0.0/0.0/16 019/0000765 ``Research Center for Informatics''.

\paragraph{Acknowledgments.} This work was supported by the Junior Star GACR GM 21-28830M; the Czech National Recovery Plan—CEDMO 2.0 NPO (MPO 60273/24/21300/21000) provided by the Ministry of Industry and Trade; the EU Horizon Europe programme MSCA PF RAVIOLI (No. 101205297) and HERON-Hellenic Robotics Center of Excellence (No. 101136568); the National Recovery and Resilience Plan “Greece 2.0”/NextGenerationEU project “Applied Research for Autonomous Robotic Systems” (MIS5200632); and Czech Technical University in Prague (SGS23/173/OHK3/3T/13 and institutional Future Fund). We acknowledge VSB – Technical University of Ostrava, IT4Innovations National Supercomputing Center, Czech Republic, for awarding this project (OPEN-33-67) access to the LUMI supercomputer, owned by the EuroHPC Joint Undertaking, hosted by CSC (Finland) and the LUMI consortium, through the Ministry of Education, Youth and Sports of the Czech Republic via the e-INFRA CZ project (ID: 90254). We also acknowledge the OP VVV project “Research Center for Informatics” (CZ.02.1.01/0.0/0.0/16 019/0000765).

==> tex/dataset.tex <==
\section{\dataset dataset}
\label{sec:dataset}

\subsection{Overview and structure}

We introduce the \emph{i}-nstance-level Composed Image Retrieval (\dataset) evaluation dataset. Following the instance-level class definition~\cite{rit+18,met_dataset}, we group all visually indistinguishable objects, \ie the same particular object, into a single class. For example, a class may correspond to (i) a concrete physical entity, such as the Temple of Poseidon, or (ii) a fictional yet visually distinctive character or object, such as Batman. In practice, if a human observer can confidently state that multiple visual manifestations represent the \emph{same object}, they belong to the same instance-level class.

Given a \emph{composed query} $(q^v,\,q^t)$ consisting of a visual query $q^v$ depicting a particular object, also referred to as an object instance or simply \emph{instance}, and a text query $q^t$ describing a modification, the goal is to rank a database of images such that those depicting the same instance under the requested modification appear at the top. We refer to these images as \emph{composed positives} or simply \emph{positives}. For each composed query, we consider the following types of hard negative images: (i) \emph{visual hard negative}: depicts an identical or visually similar object as $q^v$ but does not match the textual modification $q^t$, (ii) \emph{textual hard negative}: matches the semantics of $q^t$ but depicts a different instance, typically from the same semantic category, (iii) \emph{composed hard negative}: nearly matches both query parts, while one of the two may be identically matched, \ie depicts an object similar/identical to $q^v$  with semantics similar to $q^t$, or an object similar to $q^v$  with semantics identical/similar to $q^t$. Examples are shown in \autoref{fig:teaser} and \autoref{fig:vis}.

All types of negatives, including non-hard ones, are treated equally during evaluation. However, we include a significant number of hard negatives in our dataset to create a challenging yet manageable benchmark that supports future research. There are $n^v$ image queries for the same instance combined with $n^t$ text queries that are combined to construct $n^v n^t$ composed queries (values of $n^v$ and $n^t$ vary per instance). Unlike typical retrieval benchmarks that use a single common database for all queries, we employ the same image database for all $n^v n^t$ composed queries of an instance, but a different database for queries of other instances. This design ensures scalable and error-free labeling, avoiding the impracticality of verifying each database image as positive or negative for every query.

%--------------------------------------------------------------------

\subsection{Collection and curation}
\label{sec:dataset_collect}

The dataset construction process combines human input with automated image retrieval\footnote{We perform \emph{image-to-image} and \emph{text-to-image} retrieval using dot product search based on image and text representations obtained from OpenAI CLIP~\cite{clip}.}. Our aim is to curate, for each instance, composed queries, sets of corresponding positives, and a well-structured set of challenging hard negatives, with all \dataset images sourced from the LAION~\cite{laion} dataset.

The process for each instance begins by defining the object instance, \eg Temple of Poseidon, and selecting semantically meaningful modifications, \eg  \texttt{``at sunset''}, while avoiding implausible ones, \eg \texttt{``with snow''}. We then create \emph{seed images} and \emph{seed sentences} to serve as queries for retrieving neighbors from LAION, which collectively form a \emph{candidate image pool} that includes potential queries, positives, and hard negatives.

% \begin{itemize}
%     \item \textbf{Seed images:} 2 to 5 high-quality images depicting (i) the object instance, \eg the Temple of Poseidon, or (ii) a composed positive, \eg the Temple of Poseidon at sunset. These images are gathered from web searches in Creative Commons repositories or personal photo collections. The neighbors retrieved from LAION are categorized as visual and composed hard negatives for cases (i) and (ii), respectively.
%     \item \textbf{Seed sentences:} Textual descriptions of (i) the instance (\eg \texttt{``Temple of Poseidon''}), (ii) another object of the same category (\eg \texttt{``Ancient Greek Temple''}), (iii) rephrased versions of defined modifications (\eg \texttt{``a photo of nightfall''}), (iv) the instance under the modifications (\eg \texttt{``Temple of Poseidon at sunset''}), (v) an object of the same semantic category under the modification (\eg \texttt{``an Ancient Greek Temple at sunset''}). The neighbors retrieved from LAION are categorized  as visual, textual and composed hard negatives for cases (i \& ii), (ii), and (iv \& v), respectively.
% \end{itemize}

\textbf{Seed images:} 2 to 5 high-quality images depicting (i) the object instance, \eg the Temple of Poseidon, or (ii) a composed positive, \eg the Temple of Poseidon at sunset. These images are gathered from web searches in Creative Commons repositories or personal photo collections. The neighbors retrieved from LAION are categorized as visual and composed hard negatives for cases (i) and (ii), respectively.

\textbf{Seed sentences:} Textual descriptions of (i) the instance (\eg \texttt{``Temple of Poseidon''}), (ii) another object of the same category (\eg \texttt{``Ancient Greek Temple''}), (iii) rephrased versions of defined modifications (\eg \texttt{``a photo of dusk''}), (iv) the instance under the modifications (\eg \texttt{``Temple of Poseidon at sunset''}), (v) an object of the same semantic category under the modification (\eg \texttt{``an Ancient Greek Temple at sunset''}). The neighbors retrieved from LAION are classified as visual, textual, and composed hard negatives for cases (i \& ii), (iii), and (iv \& v), respectively.


After building the candidate image pool, automated filtering removes low-resolution, watermarked, or duplicate content using perceptual hashing and resolution checks. Annotators then manually inspect the remaining images to identify composed \emph{positives} per composed query.
% most of which come from the set of composed hard negatives, though other categories may also contain positives.
Unmarked images are considered \emph{negatives}. \emph{Visual hard negatives} are associated with all composed queries of an instance, while \emph{textual} and \emph{composed hard negatives} are associated only with the specific composed query from which (or from whose text query) they were derived. Finally, annotators manually select images within the visual hard negatives to serve as \emph{image queries}. All images that were neither filtered out from the candidate image pool nor selected as queries form the database for this instance. Positives and hard negatives associated with a composed query are negatives for another composed query.

To avoid bias towards/against CLIP-based methods, seed images are discarded and not included in \dataset, while seed sentences do not include the exact phrasing of a text query.

%--------------------------------------------------------------------
\begin{figure}[t]
\vspace{-20pt}
    \vfill
    \centering
    \scalebox{1}{
    \begin{tabular}{cccc}
        \begin{subfigure}{0.25\textwidth}
            \centering
            \input{fig/dist_query_imgs_per_instance}
            %\caption{}
        \end{subfigure}
        \hspace{-16pt}
        &
        \begin{subfigure}{0.25\textwidth}
            \centering
            \input{fig/dist_text_queries_per_instance}
            %\caption{}
        \end{subfigure}
        \hspace{-16pt}
        &
        \begin{subfigure}{0.25\textwidth}
            \centering
            \input{fig/dist_hard_negatives_per_instance}
            %\caption{}
        \end{subfigure}
        \hspace{-16pt}
        &
        \begin{subfigure}{0.25\textwidth}
            \centering
            \input{fig/dist_pos_imgs_per_query}
            %\caption{}
        \end{subfigure}
    \end{tabular}
    }
    \vspace{-10pt}
    \caption{\emph{\dataset statistics}. From left to right: Number of (a) image queries, (b) text queries, and (c) hard negatives per instance; (d) positives per composed query.
    \label{fig:stats}
    %
    \vspace{-15pt}
    }
    %
\end{figure}
%--------------------------------------------------------------------

% \subsection{Overview}

% We introduce \emph{i}-nstance–level Composed Image Retrieval (\dataset) benchmark dataset. Following an instance‑level class definition~\cite{rit+18,met_dataset}, we treat all visually indistinguishable depictions of the same identity as one class. The identity can be (i) a concrete physical entity—\eg Temple of Poseidon—or (ii) a fictional yet visually canonical character or object—\eg Batman. In practice, if a human observer would confidently say “this is the \emph{same thing}’’ across multiple visual manifestations, then these belong to the same instance class.

% Given a \emph{composed query} $(q^v,\,q^t)$—an image $q^v$ depicting an instance and a textual modification $q^t$—the goal is to rank a database of images so that images of the \emph{same instance under the requested modification} appear at the top. We call these images \emph{composed positives} or simply \emph{positives} (\autoref{fig:teaser}). For every composed query we label each non‑positive database image as one of the following: (i) \emph{visual hard negative}: depicts the same instance as $q^v$ but fails the textual modification $q^t$, (ii) \emph{textual hard negative}: satisfies $q^t$ yet shows a different instance, (iii) \emph{composed hard negative}: appears to satisfy both the identity and the modification according to a quick glance, but on closer inspection breaks either requirement—\eg a monochrome engraving of the right temple instead of an old archival photo, or an aerial shot of a visually similar temple. All remaining images—those unrelated to either the instance or the modification—are labelled simply \emph{negatives} or \emph{distractors}. To prevent degenerate matches we further impose a view‑overlap constraint: a database image is considered positive only when at least one surface patch visible in the query image is also visible in the candidate view.

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{fig/i_cir.pdf}
%     \caption{\emph{Illustration of \dataset}. Each instance consists of a set of query images and query texts, which are combined to form composed queries simulating realistic retrieval intents. For each composed query, the database includes composed positives that depict the same instance as the query image, modified according to the query text. Additionally, the database contains three categories of hard negatives: visual hard negatives (same or similar instance, different text), textual hard negatives (different instance, fully or matching text), and composed hard negatives (misleading combinations of both).}
%     \label{fig:dataset}
% \end{figure}


% \begin{figure}[t]
%     \vfill
%     \centering
%     \scalebox{1.5}{
%     \begin{tabular}{ccc}
%         \hspace{-25pt}
%         \begin{subfigure}{0.22\textwidth}
%             \centering
%             \input{fig/dist_query_imgs_per_instance}
%             \vspace{-5pt}
%             \caption{\label{fig:dist_pos}}
%         \end{subfigure}
%         &
%         \hspace{-40pt}
%         \begin{subfigure}{0.22\textwidth}
%             \centering
%             \input{fig/dist_query_imgs_per_instance}
%             \vspace{-5pt}
%             \caption{\label{fig:dist_seg}}
%         \end{subfigure}
%         &
%         \hspace{-45pt}
%         \begin{subfigure}{0.22\textwidth}
%             \centering
%             \input{fig/dist_query_imgs_per_instance}
%             \vspace{-5pt}
%             \caption{\label{fig:dist_scale}}
%         \end{subfigure}
%     \end{tabular}
%     }
%     \vspace{-15pt}
%     \caption{\textbf{\ours statistics}. (a) number of positives per object, (b) positive distribution by the SAM segments outside the bounding box, (c) image distribution by the relative bounding box area.
%     \label{fig:statistics}
%     %
%     \vspace{-15pt}
%     }
%     %
% \end{figure}



% \subsection{Collection and Curation}

% Constructing the ILCIR dataset involves a two-stage human-in-the-loop pipeline that combines human insight with automated \emph{image-to-image} and \emph{text-to-image} retrieval in LAION~\cite{laion}. The goal is to curate, for each instance, composed queries, sets of corresponding positives, and a clean, challenging set of hard negatives. This process is carried out by two groups: a team of researchers, referred to as \emph{collectors}, and a separate group of trained \textit{annotators}, each with distinct responsibilities.

% Each instance begins with the selection of a real-world or fictional concept, such as the ``Temple of Poseidon''. Collectors first define semantically meaningful modifications (\eg \texttt{``at sunset''}) and avoid modifications that may be implausible (\eg \texttt{``with snow''}). Then, they gather the LAION retrieval inputs:

% \begin{itemize}
%     \item For image-to-image retrieval, they collect 2--5 high-quality, Creative Commons or personal \emph{photos} of (i) the instance and (ii) each composed positive (\eg Temple of Poseidon at sunset). These images are used to retrieve candidates from LAION via OpenAI CLIP~\cite{clip} but are not part of the ILCIR dataset.
%     \item For text-to-image retrieval, they write a variety of \emph{textual prompts}: instance descriptions (e.g., \texttt{``Temple of Poseidon''}), composed positive forms (e.g., \texttt{``Temple of Poseidon at sunset''}), composed hard negative forms (e.g., \texttt{``an Ancient Greek Temple at sunset''}), visual hard negative forms (e.g., \texttt{``Ancient Greek Temple''}), and textual hard negative forms (e.g., \texttt{``sunset photo''}).
% \end{itemize}

% Retrieved results populate the pool of potential query images, positives, and hard negatives of the ILCIR dataset. Failure cases—such as retrieving \textit{Acropolis of Athens} images—serve as natural hard negatives. Similarly, retrieving \textit{Acropolis at sunset} when searching for \textit{Temple of Poseidon at sunset} yields composed hard negatives. All retrieved images undergo automated filtering to remove low-resolution, watermarked, or duplicate content using perceptual hashing and resolution checks.

% Collectors then manually select one or more final query images and composed positives, distinct from any Google-sourced or input images. Text queries may also be rephrased to prevent textual overlap with retrieval inputs. To isolate hard negatives, the remaining pool is reviewed by the annotators. Given visual examples of valid compositions, annotators exhaustively remove any remaining positives. Only visually or semantically similar but incorrect images are retained as hard negatives. Irrelevant or inappropriate content is discarded entirely.

% For scalability and consistency, ILCIR uses an \emph{instance-specific database design}: each instance has its own retrieval pool and annotated database. While sharing a unified negative pool across all instances may seem cleaner, it introduces significant annotation overhead and undermines per-instance semantic integrity—especially in closely related cases (e.g., \textit{Batman} vs. \textit{Batmobile}). The result is a dataset that emphasizes compositionality and specificity. Each instance is paired with a precise composed query and an annotated database of curated positives and negatives, enabling robust evaluation of instance-level composed image retrieval.

% -------------------------------------------------------------
\subsection{Statistics and visualisations}
% -------------------------------------------------------------

\autoref{fig:stats} summarizes per‐instance and per‐query statistics in \dataset.  We include 202 object instances and 750\,K images in total. Each instance has 1–46 image queries (195 with $>$1, median: 6) and 1–5 text modifications (median: 2), yielding 1,883 composed queries overall. Queries can be categorized either by their visual part (the object instance) or by their textual part (the modification). Each composed query has 1–127 positives (median: 5) and each instance’s database contains 951–10,045 hard negatives (median: 3,420), creating a challenging retrieval benchmark. \autoref{fig:vis} illustrates a set of randomly chosen pairings from the categorization: for each of eight visual–textual category combinations, we show the image query, composed positive, visual hard negative, textual hard negative, and composed hard negative.  These visualisations highlight the rich diversity of \dataset, both in terms of the wide array of visual categories (\eg landmarks, products, fictional characters, tech gadgets) and the broad spectrum of textual modifications (\eg viewpoints, attributes, contexts, additions), setting \dataset apart from existing CIR datasets. More info in the supplementary material.

%Appendix (\autoref{sec:datastructure}).

\input{fig/fig_qualitative}

%--------------------------------------------------------------------
\subsection{Shortcomings of existing benchmarks}
%{Why Existing Benchmarks Fall Short}

Commonly used CIR datasets include CIRR~\cite{cirr}, FashionIQ~\cite{fashioniq}, CIRCO~\cite{searle}, and ImageNet-R~\cite{imagenet_r}. CIRR, FashionIQ, and CIRCO share a common limitation: their construction relies on an automated process to select two similar images, guided by either textual or visual similarity. These images form the image query and the positive pair. Due to the nature of the image sources, either there is no obvious relation of such selected pairs or the relationship is typically at semantic level only, rather than at instance level. Subsequently, a language-based description is generated to capture the difference between the two images. However, the lack of concrete differences between the images, often coupled with their low relevance, results in descriptions that are either poor representations of meaningful text queries or inadequate components of a composed query. In many cases, the text query alone suffices to describe the positive image (\autoref{fig:modality_bias}), making the image query redundant. Moreover, these datasets exhibit a paucity of challenging negatives and a substantial rate of false negatives in their ground-truth annotations~\cite{searle}, inflating reported performance. We present such cases in the supplementary material.

%Appendix (\autoref{sec:datashortcomings}). 

Domain-conversion benchmarks such as ImageNet-R~\cite{imagenet_r}, NICO++~\cite{nico++}, and MiniDomainNet (MiniDN)~\cite{minidomainnet} extend CIR to style or context shifts (\eg \texttt{``photo''}→\texttt{``cartoon''}) but define positives by semantic class membership rather than object identity, lacking instance-level granularity. LTLL~\cite{leuven} is the sole existing instance-level domain-conversion dataset, but it is extremely limited in scale (500 images of 25 locations, two domains) and provides only binary \texttt{“archive”} \vs.\ \texttt{“today”} modifications. Furthermore, these benchmarks offer very narrow categorical variation—FashionIQ is confined to fashion items, LTLL to a two-way temporal shift, and the domain sets to domain changes only. These semantic-level definitions, small scale, minimal textual variation, and weak negative mining in prior benchmarks motivate the creation of \dataset.  

% Commonly used CIR datasets are CIRR~\cite{}, FashionIQ~\cite{}, CIRCO~\cite{} and ImageNet-R~\cite{}.
% CIRR, FashionIQ and CIRCO all suffer from the following short-coming.
% Two similar images are chosen in an automated, textual or visual similarity-guided way.
% These form the image query and the positive image.
% Due to the image sources uses, the two images have a semantic-level relation, if any, but not an instance-level one.
% Then, a language-based description of their difference is provided.
% The lack of concrete differences among the two images and the often low relevance between the two images, make the provided descriptions a poor example of a meaningful text query or a poor part of a composed query.
% It is often the case that the text query is solely able to describe the positive, without any use of the image query.
% \alert{We present such cases in the supplementary material.}

% The CIR benchmark that uses ImageNet is performing domain conversion, \eg from photographs to cartoons, using semantic-level class definition as well. The creators of this benchmark identify that the lack of datasets defined at instance-level is a limitation.
% Other CIR datasets for domain conversion~\cite{??} are created using NICO,  MiniDomainNet, and LTLL.
% The first two are at semantic-levevel, while the last one at instance-level but is rather small scale and has objects from a single domain only and two textual modifications.

% Class‑level CIR datasets were not designed for instance specificity.  Figure~\ref{fig:critique} visualises typical failure modes:

% \begin{enumerate}
%     \item \textbf{Image modality redundancy}: text alone is sufficient; the image contributes no unique signal.
%     \item \textbf{Weak visual grounding}: queries seldom require fine‑grained geometry, texture, or layout.
%     \item \textbf{Synthetic or low‑quality targets}: watermarks, clip‑art, and copyright violations are common.
%     \item \textbf{Retro‑fitted semantics}: pairs are formed post‑hoc, leading to contrived ``modifications'' that do not occur naturally.
% \end{enumerate}

% These issues limit real‑world applicability—for instance, searching one’s personal photo archive for “my \emph{own} dog, but at the beach.”
% addresses these gaps by enforcing instance‑level supervision, rigorous cleaning, and human‑validated hard negatives.



==> tex/defn.tex <==
%--------------------------------------------------------------------------------
% COLOR-CODING COMMENTS

\newcommand{\gt}[1]{{\color{green}{GT: #1}}}
\newcommand{\gtt}[1]{{\color{green}{#1}}}
\newcommand{\gtr}[2]{{\color{green}\st{#1} {#2}}}

\newcommand{\bp}[1]{{\color{purple}{BP: #1}}}
\newcommand{\bpt}[1]{{\color{purple}{#1}}}
\newcommand{\bpr}[2]{{\color{purple}\st{#1} {#2}}}

\newcommand{\ia}[1]{{\color{blue}{YA: #1}}}
\newcommand{\iat}[1]{{\color{blue}{#1}}}
\newcommand{\iar}[2]{{\color{blue}\st{#1} {#2}}}

\newcommand{\gkzt}[1]{{\color{cyan}{#1}}}
\newcommand{\gkzr}[2]{{\color{cyan}\st{#1} {#2}}}

%--------------------------------------------------------------------------------
% functions

\newcommand{\relu}{\operatorname{relu}}
\newcommand{\NN}{\operatorname{NN}}
\newcommand{\nn}[1]{\ensuremath{\text{NN}_{#1}}\xspace}
\newcommand{\knn}{\ensuremath{\text{kNN}}\xspace}

%--------------------------------------------------------------------------------
% Method macros

\newcommand{\ours}{\textsc{basic}\xspace}
\newcommand{\freedom}{FreeDom\xspace} % our method's acronym
\newcommand{\picword}{Pic2Word\xspace}
\newcommand{\searle}{SEARLE\xspace}
\newcommand{\searlexl}{SEARLE\xspace}
\newcommand{\compodiff}{CompoDiff\xspace}
\newcommand{\cirevl}{{CIReVL}\xspace}
\newcommand{\weicom}{WeiCom\xspace}
\newcommand{\magiclens}{MagicLens\xspace}
\newcommand{\covr}{CoVR-2\xspace}
\newcommand{\mcl}{MCL\xspace}

%\newcommand{\ours}{\textsc{FreeDom}\xspace}
%\newcommand{\ours}{\textsc{FreeDom}\xspace}

%--------------------------------------------------------------------------------
% Dataset macros

\newcommand{\dataset}{{\emph{i}-CIR}\xspace}
\newcommand{\imagenet}{{ImageNet-1k}\xspace}
\newcommand{\imagenetr}{{Image\-Net-R}\xspace}
\newcommand{\minidn}{{MiniDN}\xspace}
%\newcommand{\minidn}{{MiniDomainNet}\xspace}
\newcommand{\nico}{{NICO++}\xspace}
\newcommand{\ltll}{{LTLL}\xspace}
\newcommand{\fashioniq}{{FashionIQ}\xspace}
\newcommand{\cirr}{{CIRR}\xspace}
\newcommand{\circo}{{CIRCO}\xspace}
\newcommand\resnet[3]{\ensuremath{\prescript{#2}{}{\mathtt{R}}{#1}_{\scriptscriptstyle #3}}\xspace}

% terms
\newcommand{\tlabel}{label\xspace}
\newcommand{\txlabel}{text label\xspace}
\newcommand{\tlabels}{labels\xspace}
\newcommand{\txlabels}{text labels\xspace}

%--------------------------------------------------------------------------------
% revisited oxford/paris

\def\roxf{$\mathcal{R}$Oxford\xspace}
\def\rox{$\mathcal{R}$Oxf\xspace}
\def\ro{$\mathcal{R}$O\xspace}
\def\rpar{$\mathcal{R}$Paris\xspace}
\def\rpa{$\mathcal{R}$Par\xspace}
\def\rp{$\mathcal{R}$P\xspace}
\def\rdis{$\mathcal{R}$1M\xspace}

%--------------------------------------------------------------------------------
% results

\newcommand{\ts}[1]{{\color{applepurple}#1}}

\definecolor{OrangeFrame}{HTML}{D79B00}
\definecolor{OliveGreen}{RGB}{85, 107, 47}
\definecolor{BrickRed}{RGB}{156, 32, 32}
\definecolor{LightSteelBlue1}{RGB}{202, 225, 255}

\definecolor{appleblue}{RGB}{80,122,255}  % Softer, muted blue
\definecolor{applepink}{RGB}{217,127,174}  % Muted, soft pink
\definecolor{appleteal}{RGB}{85,163,152}  % Soft, calming teal
\definecolor{applepurple}{RGB}{138,107,221}  % Muted, soft purple
\definecolor{applemustard}{RGB}{234,179,77}  % Warm, soft mustard yellow
\definecolor{appleorange}{RGB}{255,127,80}  % Vibrant, distinctive orange
\definecolor{applegreen}{RGB}{52,199,89}
\definecolor{appleyellow}{RGB}{255,204,0}


%--------------------------------------------------------------------------------
\makeatletter
\newcommand\minuscule{\@setfontsize\minuscule{6}{6.2}} % text,  baseline
\makeatother

% Subset notation (readable in prose and tables)
\newcommand{\datasetNamed}{\dataset\textsubscript{named}}
\newcommand{\datasetDescriptive}{\dataset\textsubscript{descriptive}}
%--------------------------------------------------------------------------------
%--------------------------------------------------------------------------------
% teaser stuff
\definecolor{imagequerycolor}{RGB}{255,140,0}

\newcommand{\imgbox}[2][]{%
  {\setlength{\fboxrule}{.8pt}%      % border thickness
   \color{imagequerycolor}%          % border colour
   \fbox{\fig[#1]{#2}}}%             % actual image (relies on your \fig macro)
}

\definecolor{textquerycolor}{rgb}{0.21,0.49,0.74}

%\newcommand{\txtbox}[1]{%
%  {\setlength{\fboxrule}{.8pt}\color{textquerycolor}%  frame colour
%   \fbox{%
%     \color{black}%              <- reset text colour
%     \parbox[c][0.08\textwidth][c]{0.15\textwidth}{%
%       \centering\footnotesize\ttfamily #1}}}}

\newcommand{\txtbox}[1]{%
  {\setlength{\fboxrule}{.8pt}\color{textquerycolor}%
   \fbox{\parbox[c][0.05\textwidth][c]{0.105\textwidth}{%
     \centering\fontsize{7pt}{7pt}\selectfont\ttfamily #1}}}}

\newcommand{\txtboxx}[1]{%
  {\setlength{\fboxrule}{.5pt}%
   \color{textquerycolor}%
   \fbox{%
     \parbox[c][0.02\textwidth][c]{0.069\textwidth}{%
       \centering
       \fontsize{4pt}{4pt}\selectfont  % <-- note the units and the \selectfont
       \ttfamily
       #1%
     }%
   }%
  }%
}

\newcommand{\txtboxxx}[1]{%
  {\setlength{\fboxrule}{.5pt}%
   \color{textquerycolor}%
   \fbox{%
     \parbox[c][0.02\textwidth][c]{0.069\textwidth}{%
       \centering
       \fontsize{3pt}{3pt}\selectfont  % <-- note the units and the \selectfont
       \ttfamily
       #1%
     }%
   }%
  }%
}

\newcommand{\txtboxxxx}[1]{%
  {\setlength{\fboxrule}{.5pt}%
   \color{textquerycolor}%
   \fbox{%
     \parbox[c][0.024\textwidth][c]{0.069\textwidth}{%
       \centering
       \fontsize{5pt}{5pt}\selectfont  % <-- note the units and the \selectfont
       \ttfamily
       #1%
     }%
   }%
  }%
}

==> tex/exp.tex <==
\section{Experiments}
\label{sec:exp}

\subsection{Experimental setup} 
\label{sec:exp_setup}

\textbf{Datasets and evaluation protocol.} We evaluate \ours on our proposed \dataset as well as four composed image retrieval benchmarks: \imagenetr, \minidn, \nico, and \ltll. Retrieval performance is measured using the standard mean Average Precision (mAP) metric. Average Precision (AP) is computed per query by averaging the precision values at the ranks of all relevant items in the retrieval list. The mean Average Precision (mAP) is then obtained by averaging AP over all queries, providing a global measure of retrieval effectiveness that accounts for the order of relevant results. For \dataset, we report the \emph{macro-mAP} over instances, defined by first computing mAP per instance and then taking the mean of these per-instance mAPs across all instances.

\textbf{Baselines and competitors.} We include four simple baselines. ``Text'' scores each database image $x^v\in X$ by $\inner{\phi^t(q^t),\,\phi^v(x^v)}$; ``Image'' scores by $\bigl\langle\phi^v(q^v),\,\phi^v(x^v)\bigr\rangle$; ``Text + Image'' combines the similarities by summation; ``Text $\times$ Image'' by product. We also benchmark \ours against state-of-the-art zero-shot composed image retrieval methods: \weicom~\cite{pke+24}, \picword~\cite{pic2word}, \compodiff~\cite{compodiff}, CIReVL~\cite{cirevl}, \searle~\cite{searle}, \mcl~\cite{mcl}, \magiclens~\cite{magiclens}, \covr~\cite{covr}, and \freedom~\cite{freedom}. All methods use CLIP with ViT-L/14~\cite{dbk+21}, whereas \compodiff employs the larger CLIP ViT-G/14.

\textbf{\ours.} For fair comparison, we also use CLIP~\cite{clip} ViT-L/14~\cite{dbk+21}.  We set $k=250$ components for PCA, $\lambda=0.1$ for the Harris criterion and $\alpha=0.2$. These values were fixed once on a small privately owned development set, named \dataset\textsubscript{dev}. The corpora $C_+$ and $C_-$ were automatically generated using ChatGPT~\cite{hurst2024gpt}. The statistics $s^v_{\min}$ and $s^t_{\min}$ were computed over a synthetically generated dataset constructed using Stable Diffusion~\cite{stablediffusion} with automatically created prompts. More details are included in the supplementary material.

%\textcolor{red}{Further details regarding the corpora construction, dataset specifications, extended benchmark results, backbone comparisons, and full implementation details are included in the supplementary material.}

% - Hyper-parameters fixed: number of components 250, Harris criterion lambda 0.1, contrastive parameter $\alpha$ 0.2. 
% - Generation of corpora. 
% - Modality Means 
% - Min-based normalization external dataset.
% Suppl. material on these.

%----------------------------------------------------------

% \subsection{MinMax Dataset Creation}
% \textcolor{red}{suppl. material?}

% For our min-based normalization scheme we need to precalculate the corresponding statistical values $s^{\text{img}}_{min}$ and $s^{\text{text}}_{min}$, taking into account both the CLIP model backbone and the subsequent projection that takes place. To this end, we first used Google Gemini to randomly generate 100 simple textual prompts (e.g., `a dog', `a calm sea') and 100 more complex ones (such as `a hidden waterfall in a lush, green jungle'). Each prompt was then used as input to the Stable Diffusion model \cite{Rombach_2022_CVPR} to generate 4 corresponding images. We processed all image-text and image-image pairs through our full pipeline with feature extraction and projection, and computed their similarity scores. These scores were then used to derive the normalization statistics $s^{\text{img}}_{min}$ and $s^{\text{text}}_{min}$.

% %----------------------------------------------------------
% % uncomment if you want SIGLIP also
% %----------------------------------------------------------
% \begin{table}[htbp]
%     \centering
%     \caption{Ablation Study Results (mAP). "Full Method" refers to the configuration with no components removed. Subsequent rows show the mAP when the specified component is removed.}
%     \label{tab:ablation_study}
%      \begin{tabular}{l|cccc|cccc}
%         \toprule
%         & \multicolumn{4}{c}{CLIP} & \multicolumn{4}{c}{SIGLIP} \\
%         \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%         Ablation Setting        & {Im.-R} & {NICO} & {MinDIN} & {LTLL} & {Im.-R} & {NICO} & {MinDIN} & {LTLL} \\
%         \midrule
%         Full Method             & \textbf{32.05}   & \textbf{31.64}  & \textbf{39.53}    & \textbf{41.51}  & \textbf{47.02}   & \textbf{29.54}  & \textbf{51.81}    & \textbf{42.02}  \\
%         %w/o Harris     & 30.61   & 29.60  & 38.85    & 40.59  & 45.14   & 27.33  & 50.32    & \textbf{42.30}  \\
%         %w/o Min-Max Sim.        & 18.83   & 14.75  & 24.67    &  4.45  & 32.75   & 18.98  & 39.93    &  2.84  \\
%         w/o Fusion (simple mult.)        &  24.50 & 22.74 & 29.65  & 19.36 & 42.17 & 26.12 & 45.05 & 21.92 \\
%         w/o Feat. Projection    & 17.31   & 13.96  & 21.22    & 22.42  & 27.21   & 18.10  & 30.46    & 27.28  \\
%         w/o Query Expansion     & 27.28   & 28.93  & 35.86    & 37.77  & 42.18   & 27.13  & 48.35    & 38.76  \\
%         w/o Contextualization   & 26.19   & 30.61  & 33.64    & 35.10  & 40.26   & 28.66  & 43.03    & 26.01  \\
%         \bottomrule
%     \end{tabular}
% \end{table}
% %----------------------------------------------------------

% %----------------------------------------------------------
% \begin{table}[htbp]
%     \centering 
%     \caption{\emph{Ablation results mAP (\%) using the OpenAI CLIP across five CIR benchmarks}. We start from the full method (\ours) and progressively remove individual components to measure their impact. Removing projection and fusion has the most significant effect. Avg: mean across benchmarks.}
%     \label{tab:ablation_study_removing_clip} % Updated label slightly
%      % Removed the second block of cccc for SIGLIP
%      \begin{tabular}{l|ccccc|c}
%         \toprule
%         % Removed the multicolumn for SIGLIP
%         removed component        & \imagenetr & \nico & \minidn & \ltll & \dataset & Avg.  \\ % Kept CLIP headers
%         \midrule
%         \ours             & \textbf{32.05}   & \textbf{31.64}  & \textbf{39.53}    & \textbf{41.51} &  \textbf{47.04} & \textbf{38.75} \\ % Removed SIGLIP data
%         \textcolor{red}{\faTimes} Harris     & 30.61   & 29.60  & 38.85    & 40.59&  46.57 & 37.64\\ % Removed SIGLIP data
%         %w/o Min-Max Sim.        & 18.83   & 14.75  & 24.67    &  4.45  \\ % Removed SIGLIP data
%         \textcolor{red}{\faTimes} Fusion (simple mult.) & 24.50 & 22.74 & 29.65  & 19.36 & 44.18 & 28.89 \\ % Removed SIGLIP data
%         \textcolor{red}{\faTimes} Feat. Projection    & 17.31   & 13.96  & 21.22    & 22.42 & 43.39 & 23.66 \\ % Removed SIGLIP data
%         \textcolor{red}{\faTimes} Query Expansion     & 27.28   & 28.93  & 35.86    & 37.77 & 47.41 & 35.85 \\ % Removed SIGLIP data
%         \textcolor{red}{\faTimes} Contextualization   & 26.19   & 30.61  & 33.64    & 35.10 & 38.23 & 32.75\\ % Removed SIGLIP data
%         \bottomrule
%     \end{tabular}
% \end{table}
% %----------------------------------------------------------

% %----------------------------------------------------------
% \begin{table}[ht]
% \centering
% \caption{\emph{Ablation results mAP (\%) using the OpenAI CLIP across five CIR benchmarks}. We start from product of similarities and progressively add each component to isolate its impact. Components like projection and contextualization contribute the most. The final row corresponds to our full method (\ours). Avg: mean across benchmarks.
% }
% \label{tab:ablation_study_adding_clip}
% \begin{tabular}{lccccc|c}
% \toprule
% added component             & \imagenetr &  \nico & \minidn  & \ltll & \dataset & Avg. \\
% \midrule
% Text $\times$ Image                                 &  7.66 &  9.26 &  9.48 & 19.78 & 23.28 & 13.89 \\
% \textcolor{ForestGreen}{\faPlus} centering         & 12.22 & 10.48 & 12.12 & 17.04 & 36.68 & 17.71 \\
% \textcolor{ForestGreen}{\faPlus} projection        & 18.01 & 19.10 & 19.92 & 16.03 & 38.71 & 22.76 \\
% \textcolor{ForestGreen}{\faPlus} q.\ expansion     & 19.76 & 20.57 & 22.06 & 13.87 & 39.00 & 23.85 \\
% \textcolor{ForestGreen}{\faPlus} context           & 24.50 & 22.74 & 29.65 & 19.36 & 45.24 & 28.70 \\
% \textcolor{ForestGreen}{\faPlus} min\ reg.         & 30.61 & 29.60 & 38.85 & 40.59 & 45.29 & 36.99 \\
% \textcolor{ForestGreen}{\faPlus} harris (\ours)     & \textbf{32.05} & \textbf{31.64} & \textbf{39.53} & \textbf{41.51} & \textbf{46.67} & \textbf{38.68} \\
% \bottomrule
% \end{tabular}
% \label{tab:add_components}
% \end{table}
% %----------------------------------------------------------

\subsection{Experimental results} 
\label{sec:exp_results}

\textbf{Per-category performance.} In~\autoref{fig:performance_barplots} we report the per-category performance of selected baselines and competitors on \dataset split by the a) primary visual  and (b) textual categories of the queries.

In~\autoref{fig:performance_barplots}(a), \ours ranks first in six of the eight visual categories, delivering particularly large margins on fictional ($47.8\%$ \vs $31.1\%$ for SEARLE), mobility (45.8\% \vs 29.3\% for MagicLens), and technology ($30.6\%$ \vs $23.0\%$ for Text × Image). It also leads on product ($33.7\%$ \vs $26.7\%$ for MagicLens), landmark ($39.3\%$ \vs $35.0\%$ for \magiclens), and art ($38.0\%$ \vs $35.0\%$ for \magiclens). The only exceptions are fashion, where MagicLens edges out at $25.6\%$ \vs $22.0\%$ for \ours, and household, where \magiclens peaks at $29.1\%$; \ours is second at $22.4\%$. In contrast, the other methods show uneven strengths. %MagicLens excels on style-heavy classes, Pic2Word is competitive on everyday objects and FreeDom holds the third place on landmarks but struggles on technical categories.

\input{tab/exp_results_all_datasets_summary}

\autoref{fig:performance_barplots}(b) further confirms the consistency of \ours. \ours dominates projection ($53.1\%$ \vs $31.1\%$ for \magiclens), appearance ($48.8\%$ \vs $36.8\%$ for \searle), and domain ($39.3\%$ \vs $31.1\%$ for \magiclens). It also leads on vewpoint ($47.8\%$ \vs $40.1\%$ for \magiclens) and attribute ($26.3\%$ \vs $24.1\%$ for \magiclens). \ours is second on context ($35.6\%$ \vs $36.4\%$ for \magiclens) and addition ($24.0\%$ \vs $28.2\%$ for \magiclens).

%----------------------------------------------------------
\begin{figure*}[t]
\vspace{-20pt}
    \centering
    \begin{subfigure}[t]{.98\textwidth}
        \centering
        \scalebox{1}{\input{fig/fig_performance_per_visual_category}}
        \vspace{-5pt}
        \caption{\emph{Visual categories.} mAP (\%) averaged over instances in the same primary‐level visual category.}
        \label{fig:performance_barplot_visual}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{.98\textwidth}
        \centering
        \scalebox{1}{\input{fig/fig_performance_per_textual_category}}
        \vspace{-5pt}
        \caption{\emph{Textual categories.} mAP (\%) averaged over instances in the same primary‐level textual category.}
        \label{fig:performance_barplot_textual}
    \end{subfigure}
    \vspace{-5pt}
    \caption{\emph{Performance comparison on \dataset per primary category of queries.} (a) Visual, (b) Textual.}
    \label{fig:performance_barplots}
    \vspace{-15pt}
\end{figure*}
%----------------------------------------------------------

\textbf{Comparison with SOTA.}
We further evaluate the performance of \ours against all considered baselines and state-of-the-art CIR methods across five datasets, including \dataset. Results are shown in \autoref{tab:sota}. As observed, \ours consistently outperforms all competing methods across the board. 
%\alert{Additionally, \ours is significantly more lightweight in terms of computational cost compared to other state-of-the-art approaches.} 
Runtime comparisons are provided in the supplementary material.


%\textcolor{red}{discussion / intuition? why others fail?}

%----------------------------------------------------------

\subsection{Ablation studies} 
\label{sec:ablation}

% Table~\ref{tab:ablation_components} provides an in-depth analysis of the components of the proposed method, their impact and their inter-connection. 
% First, we can see that the mean centering operation provides non-trivial boost in all cases, except the LTLL dataset. 
% LTLL is the only dataset with very "strict" subject domain, describing only landmarks. 
% %Thus removing a generic mean, taken from LAION,  may not help further enhance semantic differences directly. 
% Notably, by simply adding the min-based normalization, along with the Harris criterion, we can see consistent performance improvement across all datasets, expect \dataset.
% The impact of these fusion steps, can be better understood through the two rows before the last, where we remove both min normalization and Harris, or Harris alone. 
% Notably, Harris always provides a performance increase, while when we remove the min normalization step we can see a significant drop in performance, highlighting the importance of balancing the two modalities.
% Moreover, contextualization plays a crucial role in integrating the text query. This can be best seen in the last row, whete contextualization is removed and the overall results suffer. 
% Finally, we have the image modality enhancements, namely semantic projection and query expansion. 

\textbf{\ours components.} 
\autoref{tab:ablation_components} presents a detailed ablation study on the contribution of each component of \ours across all evaluated datasets. Starting with a simple Text$\times$Image baseline, we progressively add the components of \ours, highlighting the cumulative benefits of each module.

\emph{Centering} provides a notable boost across most datasets (17.48\% $\rightarrow$ 28.33\% on \dataset) with the exception of \ltll, likely due to its narrow focus on landmarks.
\emph{Normalization and Harris fusion} further enhance retrieval, as demonstrated by their removal, 
%(rows 8, 9)
with min normalization being especially critical, since its absence causes a significant drop. Harris consistently contributes moderate gains.
\emph{Text contextualization} is also important. Its removal results in a substantial performance decline, particularly on datasets requiring nuanced language understanding (31.64\% $\rightarrow$ 25.85\% on \dataset).
On the image side, \emph{semantic projection} accounts for the majority of the performance gain in many cases, serving as a key enhancement. \emph{Query expansion} offers additional improvements, particularly on category-level datasets, though it leads to performance decrease in \dataset.
Note that some components depend on the presence of others to be effective (\eg projection assumes centered features, Harris step requires min-normalized scores).  

% \emph{Centering} provides a notable boost across most datasets with the exception of \ltll, likely due to its narrow focus on landmarks.
% \emph{Normalization and Harris Fusion} further improves retrieval performance consistently, better captured by their removal (8th and 9th rows) with min normalization emerging as especially critical: its removal leads to a significant drop, underscoring its role in balancing modalities. Harris offers steady improvements when included.
% Text \emph{contextualization} proves essential, with its removal (last row) degrading performance across the board, especially on datasets requiring nuanced language understanding.
% On the image side, \emph{semantic projection} accounts for the majority of the performance gain in many cases, serving as a key enhancement. \emph{Query expansion} offers additional improvements, particularly on category-level datasets, though it leads into negligible performance decrease in \dataset.


% It is interesting to observe the different performance gains across datasets. Regularization may be critical if the two modalities start to diverge in range significantly (LTLL) or it may provide a minor boost when the two modalities have close range as in \dataset. Contextualization does not provide the same increase for MiniDN as with the other datasets. Here we have domains noted as "rock", "water", "outdors". COntextualizing with a subject, i.e. "rock dog" or "dog rock", does not provide as meaningful represenations as in \dataset for example ("dog during sunset").

% MAYBE this BELOW FOR SUPPL
% It is interesting to observe that performance gains vary across datasets. For example, contextualization shows limited benefit on MiniDN, where domain labels like ``rock'', ``water'', ``outdoors'' add little when combined with subjects (e.g., ``rock dog''). In contrast, contextualized phrases in \dataset, such as ``dog during sunset'', yield richer representations.

%----------------------------------------------------------
% Option: Cumulative table WITHOUT a descriptive first column
%----------------------------------------------------------
\begin{table}[!t]
\centering
\caption{Ablation study reporting average mAP (\%) across datasets. Each row progressively adds or removes components of the proposed method: mean centering (\textit{Centering}), min-based normalization (\textit{Min Norm.}), Harris criterion (\textit{Harris}), text contextualization (\textit{Context.}), semantic projection (\textit{Proj.}), and query expansion (\textit{Q. Exp.}). 
%The final five columns report performance across individual datasets, while the progression of rows allows assessment of component-wise contributions.
The first row (no component applied) corresponds to Text $\times$ Image.
}
\label{tab:ablation_components}
\resizebox{.98\textwidth}{!}{%
\begin{tabular}{cccccc ccccc} % No 'l' at the beginning
\toprule
% \rotcol{Centering} & \rotcol{Min. Reg.} & \rotcol{Harris} & \rotcol{Context.} & \rotcol{Proj.} & \rotcol{Q. Exp.} & \imagenetr & \nico & \minidn & \ltll & \dataset & \textbf{Avg.} \\
{Centering} & {Min Norm.} & {Harris} & {Context.} & {Proj.} & {Q. Exp.} & \imagenetr & \nico & \minidn & \ltll & \dataset \\ % & \textbf{Avg.} \\
\midrule
\Crs  & \Crs  & \Crs  & \Crs  & \Crs  & \Crs  &  7.66 &  9.26 &  9.48 & 19.78 & 17.48 \\ % & 13.89 \\
\Tck  & \Crs  & \Crs  & \Crs  & \Crs  & \Crs  & 12.16 &  9.95 & 12.16 & 16.93 & 28.33 \\ % & 17.65 \\
\Tck  & \Tck  & \Crs  & \Crs  & \Crs  & \Crs  & 12.06 & 17.20 & 17.72 & 22.20 & 27.30 \\ % & 20.43 \\  
\Tck  & \Tck  & \Tck  & \Crs  & \Crs  & \Crs  & 16.21 & 15.06 & 17.79 & 29.70 & 28.42 \\ % & 23.10 \\
\Tck  & \Tck  & \Tck  & \Tck  & \Crs  & \Crs  & 18.61 & 15.34 & 21.01 & 33.74 & 33.48 \\ % & 26.29 \\
\Tck  & \Tck  & \Tck  & \Tck  & \Tck  & \Crs  & 27.54 & 28.90 & 35.75 & 38.22 & \textbf{34.35} \\ % & 35.63 \\
%\hdashline
\midrule
\Tck  & \Tck  & \Tck  & \Tck  & \Crs   & \Tck  & 17.31  & 13.96  & 21.22  & 22.42  & 31.78 \\
\Tck  & \Tck  & \Tck  & \Crs   & \Tck  & \Tck  & 26.18  & 30.61  & 33.64  & 34.50 & 25.85 \\
\Tck  & \Tck  & \Crs   & \Tck  & \Tck  & \Tck  & 30.75  & 29.82  & 38.85  & 40.65 & 31.61 \\
%\Tck  & \Crs   & \Tck  & \Tck  & \Tck  & \Tck  & 18.83  & 19.93  & 24.67  & 4.36 & 27.87 \\
%\Crs  & \Tck  & \Tck  & \Tck  & \Tck  & \Tck  & 23.29 & 19.93 & 24.87 & 10.16 & 12.65 \\
%\midrule
%\Crs  & \Crs  & \Tck  & \Tck  & \Tck  & \Tck  & 26.48 & 24.88 & 33.45 & 32.66 & 26.63 \\
\Tck  & \Crs  & \Crs  & \Tck  & \Tck  & \Tck  & 24.50 & 22.74  & 29.65  & 19.36 & 30.75 \\
\midrule
\Tck  & \Tck  & \Tck  & \Tck  & \Tck  & \Tck  & \textbf{32.13} & \textbf{31.65} & \textbf{39.58} & \textbf{41.38} & 31.64 \\ % & \textbf{38.43} \\
%\hdashline

%\Tck  & \Tck  & \Crs  & \Tck  & \Tck  & \Tck  & 30.75  & 29.82 & 38.85 & 40.65  & 46.11 \\
%\Tck  & \Tck  & \Tck  & \Crs  & \Tck  & \Tck  & 26.18 & 30.61 & 33.64 & 34.50 &  39.74 \\



%\Tck & \Crs  & \Tck  & \Tck  & \Tck  & \Tck  & 18.83 & 19.93 & 24.67 & 4.36 & 42.14 \\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{table}
%----------------------------------------------------------

% %----------------------------------------------------------
% \begin{table}[ht]
% \centering
% \caption{\emph{Ablation results mAP (\%) using the OpenAI CLIP across five CIR benchmarks}. We start from product of similarities and progressively add each component to isolate its impact. Components like projection and contextualization contribute the most. The final row corresponds to our full method (\ours). Avg: mean across benchmarks.
% }
% \label{tab:ablation_study_adding_clip}
% \resizebox{.49\textwidth}{!}{
% \begin{tabular}{lccccc}
% \toprule
% added component             & \imagenetr &  \nico & \minidn  & \ltll & \dataset \\
% \midrule
% Text $\times$ Image                                 &  7.66 &  9.26 &  9.48 & 19.78 & 23.28 \\
% \textcolor{ForestGreen}{\faPlus} centering         & 12.16 & 9.95 & 12.16 & 16.93 & 37.05 \\
% \textcolor{ForestGreen}{\faPlus} min. reg & 12.06  & 17.20 & 17.72 & 22.20 & 32.98 \\  
% \textcolor{ForestGreen}{\faPlus} harris & 16.21 & 15.06 & 17.79 & 29.70 & 36.76\\
% \textcolor{ForestGreen}{\faPlus} context & 18.61 & 15.34 & 21.01 & 33.74 & 42.74 \\
% \textcolor{ForestGreen}{\faPlus} projection & 27.54 & 28.90 & 35.75 & 38.22 & 47.73\\
% \textcolor{ForestGreen}{\faPlus} q. expansion (\ours) & 32.13 & 31.65 & 39.58 & 41.38 & 47.39 \\
% \bottomrule
% \end{tabular}
% }
% \resizebox{.49\textwidth}{!}{
% \begin{tabular}{lccccc}
% \toprule
% added component             & \imagenetr &  \nico & \minidn  & \ltll & \dataset \\
% \midrule
% Text $\times$ Image                                 &  7.66 &  9.26 &  9.48 & 19.78 & 23.28 \\
% \textcolor{ForestGreen}{\faPlus} centering         & 12.22 & 10.48 & 12.12 & 17.04 & 36.68 \\
% \textcolor{ForestGreen}{\faPlus} projection        & 18.01 & 19.10 & 19.92 & 16.03 & 38.71 \\
% \textcolor{ForestGreen}{\faPlus} q.\ expansion     & 19.76 & 20.57 & 22.06 & 13.87 & 39.00 \\
% \textcolor{ForestGreen}{\faPlus} context           & 24.50 & 22.74 & 29.65 & 19.36 & 45.24 \\
% \textcolor{ForestGreen}{\faPlus} min\ reg.         & 30.75 & 29.82 & 38.85 & 40.64 & 46.11 \\
% \textcolor{ForestGreen}{\faPlus} harris (\ours)     & \textbf{32.13} & \textbf{31.65} & \textbf{39.58} & \textbf{41.38} & \textbf{47.39}  \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:add_components}
% \end{table}
%----------------------------------------------------------

%\textbf{Controlling Semantic Projection.}

%----------------------------------------------------------
% \begin{table}[ht]
% \centering
% \scriptsize
% \begin{tabular}{l|cc|cccc}
% \toprule
% Dataset / Negative Corpus & none  & generic & ImagenetR & LTLL  & MINIDN & NICO  \\
% \midrule
% ImagenetR                  & 30.15 & 32.05   & \textbf{33.22}     & 30.74 & 31.21  & 30.79 \\
% LTLL                       & 41.80 & 41.51   & 41.33     & \textbf{44.09} & 42.13  & 43.48 \\
% MINIDN                     & 38.64 & 39.53   & 39.38     & 38.72 & \textbf{39.60}  & 38.76 \\
% NICO                       & 30.67 & 31.64   & 30.84     & 31.20 & 30.67  & \textbf{31.17} \\
% \bottomrule
% \end{tabular}
% \caption{Accuracy (\%) on each dataset using different negative corpora.}
% \label{tab:negative-corpus-results}
% \end{table}

% \begin{table}[ht]
% \centering
% \scriptsize
% \caption{mAP(\%) on each dataset using different negative corpora. The first column lists the evaluation datasets. The top row specifies the source of the negative corpus used for training/evaluation.}
% \begin{tabular}{l | c c | c c c c}
% \toprule

% \multicolumn{1}{c|}{} & \multicolumn{6}{c}{Negative Corpora Source} \\ 
% \cmidrule(lr){2-7}

% Evaluation Dataset &
%   none &
%   \multicolumn{1}{c|}{generic} &
%   Imagenet-R &
%   LTLL &
%   MiniDN &
%   NICO++ \\
% \midrule
% % Data rows - the dataset names are now in the first column
% Imagenet-R & 30.15 & 32.05 & \textbf{33.22} & 30.74 & 31.21 & 30.79 \\
% LTLL      & 41.80 & 41.51 & 41.33          & \textbf{44.09} & 42.13 & 43.48 \\
% MiniDN    & 38.64 & 39.53 & 39.38          & 38.72          & \textbf{39.60} & 38.76 \\
% NICO++      & 30.67 & \textbf{31.64} & 30.84          & 31.20          & 30.67          & 31.17 \\
% \dataset & 46.62 & \textbf{47.39} & 46.43 & 47.15 & 46.24 & 46.52 \\
% \bottomrule
% \end{tabular}
% \label{tab:negative-corpus-results-simple-header}
% \end{table}

\begin{wraptable}{l}{0.52\textwidth}
\vspace{-10pt}
%\begin{table}[ht]
\centering
%\scriptsize
\setlength{\tabcolsep}{3pt}      % tighten inter-column padding
\renewcommand{\arraystretch}{0.9} % tighten row spacing
\caption{mAP(\%) on each dataset using different negative corpora. The first column lists the evaluation datasets.}
\label{tab:neg-corpus-impact}
\resizebox{.52\textwidth}{!}{
\begin{tabular}{@{}lcccccc@{}}
\toprule
 & \multicolumn{6}{c}{Negative~Corpora~Source}\\
\cmidrule{2-7}
Eval.~Dataset & none & generic & Imagenet-R & NICO++ & MiniDN & LTLL\\
\midrule
Imagenet-R & 30.15 & 32.13 & \textbf{33.22} & 30.74 & 31.17 & 30.91\\
NICO++     & 30.67 & \textbf{31.65} & 30.84          & 31.17 & 30.67 & 31.20\\
MiniDN     & 38.64 & 39.38          & 39.34          & 38.75 & \textbf{39.58} & 38.68\\
LTLL       & 41.80 & 41.24          & 41.33          & 43.39 & 42.09 & \textbf{43.98}\\
%\dataset   & 46.62 & \textbf{47.39} & 46.43          & 46.52 & 46.24 & 47.15\\
\dataset   & 31.51 & \textbf{31.64} & 31.61          & 31.20 & 31.32 & 31.06\\
\bottomrule
\end{tabular}
}
\vspace{-5pt}
%\end{table}
\end{wraptable}

%\textbf{Controlling Semantic Projection} \autoref{tab:neg-corpus-impact} includes what happens when we omit $C_-$, use a generic negative corpus, or use a dataset-specific corpus, attained through ChatGPT, that tries to capture the domain variability of \imagenetr, \nico, \minidn and \ltll. We can see that known biases of the datasets can further improve performance, especially when compared to the case where no $C_-$ is used. This concept will be further explored in the supplementary material.

\textbf{Controlling semantic projection.} \autoref{tab:neg-corpus-impact} shows the effect of omitting $C_-$, using a generic negative corpus, or using a dataset-specific corpus (generated via ChatGPT) designed to reflect the domain variability of \imagenetr, \nico, \minidn, and \ltll. Results indicate that leveraging 
% known dataset biases 
application-related knowledge
can improve performance, particularly compared to omitting $C_-$. This idea is further discussed in the supplementary material.

\textbf{\dataset: Compact but hard.} 
We use randomly selected images from LAION as negatives to assess how challenging \dataset is in comparison to a large-scale database that is commonly shared across all queries and lacks explicit hard negatives. 
Using the performance of Text $\times$ Image baseline as a reference (17.48\%), we find that more than 40M distractor images are required for this baseline to reach a similarly low performance. 
Note that the performance measured using unlabeled LAION images as negatives is only a lower bound because of the inevitable presence of false negatives.
This is four orders of magnitude larger than the 3.7K database images per query, on average, that \dataset uses, or 1.5 orders of magnitude larger than the 750K database images used among all queries; the latter defines the experimental processing cost.
More analysis is provided in the supplementary material.  

\textbf{\dataset: Truly compositional.} A dataset that requires \emph{composition} should reward combining text and image, not either modality alone. To diagnose this, we sweep a mixing weight $\lambda\!\in\![0,1]$ between text-only ($\lambda{=}0$) and image-only ($\lambda{=}1$) similarity for three simple fusion methods (\weicom, Text $+$ Image, Text $\times$ Image), and plot mAP as a function of $\lambda$ (\autoref{fig:modality_bias}). For each method we compute the \emph{composition gain} $\Delta$: the difference between the peak value of the curve and the best uni-modal endpoint, and then average $\Delta$ across the three methods. On \dataset, the average composition gain is large: $+14.9$ mAP ($+490\%$ relative to the best uni-modal baseline), with peaks occurring at interior $\lambda$—clear evidence that both modalities must work together. By contrast, it shrinks to $+3.0$ mAP ($+11\%$) on \cirr, $+5.0$ mAP ($+26\%$) on \fashioniq, and $+6.8$ mAP ($+167\%$) on \circo. Moreover, the highest uni-modal performance of \cirr and \fashioniq is always when ($\lambda = 0$), \ie text-only. Thus legacy datasets reward composition only marginally, whereas \dataset demands genuine cross-modal synergy; BASIC is designed for the latter scenario. 

\begin{figure}[t]
\centering
\vspace{-20pt}
\input{fig/fig_bias}
\vspace{-5pt}
\caption{\emph{Modality bias via weight sweeps.} mAP(\%) \vs \ fusion weight $\lambda$ for three simple methods, where $\lambda{=}0$ is text-only and $\lambda{=}1$ is image-only. Compositional datasets should peak at interior $\lambda$ and exceed both endpoints. \dataset{} shows strong interior optima and large gains over the best uni-modal baseline; CIRR and FashionIQ peak at $\lambda{=}0$, indicating text dominance.}
\label{fig:modality_bias}
\end{figure}

% Replacing the 300k curated hard negatives of \dataset with 300k random LAION~\cite{laion} distractor images inflates the Text $\times$ baseline mAP from 23.28 \% to 88.57 \%; roughly 20M distractors would be required to recover the original 23.28\% mAP. More ablations are provided in the supplementary material.  

% TODO: HARD NEGATIVES

%\begin{wrapfigure}{r}{0.45\linewidth}  % 'r' for right side, width=45% of text
%  \centering
%  \input{fig/fig_ablation_laion_distractors}
  %\caption{Extrapolated mAP / mMAP vs.\ random LAION distractors.}
%  \label{fig:distractors}
%\end{wrapfigure}



%\textbf{Impact of Hard Negatives.}
%Finally, we compare our curated hard negatives against random LAION distractors of varying sizes.  As shown in \autoref{fig:distractors}, replacing the 300 K–image database with $\approx$20 M random images yields almost identical mAP and mMAP to our original setup (20.78 % and 23.28 %, respectively), demonstrating that our targeted hard‐negative curation produces a compact yet equally challenging benchmark (see Supplementary Sec.~X for details).






%----------------------------------------------------------


==> tex/intro.tex <==
\section{Introduction}
\label{sec:intro}

\emph{Composed image retrieval} (CIR) combines image-to-image retrieval and text-to-image retrieval. CIR uses a composed query, \ie an image and text, to retrieve images whose content matches both the visual and textual parts of the query. Vision and language models (VLMs)~\cite{clip, blip, blip2, align, siglip} provide the foundation for developing CIR methods, either through further training~\cite{cirr, fashionvlp, combiner, liu2024bi} or in a training-free manner~\cite{pke+24, freedom, cirevl}. The use of VLMs, owing to their large-scale pre-training, enables CIR to operate in an open-world setting and compare any kind of visual or textual content. This capability paves the way for novel applications and advanced methods to explore and browse large image collections. However, the main limitation of CIR lies in the lack of appropriate data for both evaluating progress and training models. This work addresses these challenges.

Existing CIR datasets~\cite{cirr,fashioniq,searle} often suffer from poor quality~\cite{searle,collm} due to their construction process, \ie two similar images are selected automatically and their difference is textually described. This approach incorrectly assumes that such a difference always forms a meaningful text query for retrieval, regardless of the image pair.
In contrast, given one image, we first specify a textual modification such that both together form a meaningful composed query. We then identify positive and a large set of hard negative images to construct \dataset, a compact yet challenging dataset. The goal is to retrieve images that depict the same object instance as the image query, under the modification described by the text query. Such an instance-level object class definition is missing from existing datasets and is identified as a limitation by prior work~\cite{pic2word}. By integrating diverse object types and modification types, \dataset accurately reflects a wide range of real-world use cases.

CIR methods that rely on further training on top of VLMs require large amounts of training triplets in the form of (query image, query text, positive image), which are challenging to obtain at scale. As a result, training is typically performed on small sets of manually labeled triplets~\cite{tirg, cirr, combiner, artemis}, or on automatically generated triplets obtained through crawling~\cite{magiclens, hycir, transagg} or synthetic data generation~\cite{compodiff}. However, these automated methods significantly compromise triplet quality, and in all cases, the diversity of visual object types and textual modifications remains limited compared to the variety present in VLM pre-training, thereby restricting generalization ability.
Instead, we develop a training-free \underline{\textsc{b}}aseline \underline{\textsc{a}}pproach for \underline{\textsc{s}}urpr\underline{\textsc{i}}singly strong \underline{\textsc{c}}omposition, \ours, which fully leverages existing VLM capabilities and remains adaptable to future advances.


\ours separately computes the similarity with respect to each query component and performs fusion inspired by the classical Harris corner principle~\cite{harris1988combined}; both responses must be jointly high, rather than just one of the two.
The image-to-image dot product similarity is enhanced through a projection computed analytically not in the image space, but in the text representation space. This is facilitated by a large language model (LLM) that provides common object names and typical textual modifications.
The aim is to increase distinctiveness regarding object variations, \ie to better represent image objects beyond other visual cues, while achieving invariance to textually described modifications, so that the same object is retrieved despite variations. Interestingly, this projection can also be equivalently applied solely on the query side, enabling user-specific or application-specific customization.
The text-to-image dot product similarity is refined via a query-time contextualization process designed to bridge the distribution gap between the text inputs seen during VLM pre-training and the text queries used at inference. Our contributions are summarized as follows:
%\ours establishes a new state of the art on \dataset and four existing CIR datasets focused on domain conversion, while maintaining efficiency and simplicity.
%
\begin{itemize}
\item We introduce \dataset, a new evaluation dataset for CIR, meant to retrieve images containing the same particular object as the visual query under modifications defined by the text query.
\item We introduce \ours, a training-free approach leveraging pre-trained VLMs for class-level or instance-level CIR that is based on image-to-image and text-to-image similarities, without the need to update the database embeddings.
\item \ours sets a new state of the art on \dataset and across existing class-level CIR datasets.
\end{itemize}

% Information retrieval from large image collections is a well-studied problem with numerous real-world applications. Among the various retrieval tasks, image-to-image retrieval involves using a visual query, \ie an image, to retrieve examples that depict visually relevant content. Relevance can be defined at different levels of granularity, ranging from the semantic level to the instance level. The latter, which focuses on retrieving particular objects, is  useful for applications such as retail product retrieval, artwork recognition, and visual localization.
% In contrast, text-to-image retrieval involves using a textual query, \ie a word, phrase, or sentence, to find examples that match the described semantics. While both retrieval types have distinct challenges, they share the goal of accurately matching the query with the most relevant content.
% Composed Image Retrieval (CIR) is a recently introduced task that uses a composed query formed by both visual and textual inputs. In this setup, the retrieved examples must jointly satisfy the visual and textual components. Typically, the textual part either modifies or supplements the visual content, providing a rich and flexible way to navigate image collections. However, current methods typically require retrieved examples to match both parts of the query at a semantic level, a significant limitation stemming from existing dataset constraints.

% In this work, we focus on Instance-Level Composed Image Retrieval (ILCIR), which we argue is the most practical and challenging variant due to its relevance to real-world applications. ILCIR requires the retrieved examples to depict the same particular object as the visual query, while the context, viewing conditions, or domain may vary according to the textual input. One of the primary challenges of ILCIR is the creation of suitable datasets, as instance-level relevance annotations are time-consuming and costly, often resulting in smaller datasets.
% To address this gap, we present the first large-scale ILCIR dataset, incorporating a diverse set of visual and textual queries. In contrast to existing dataset, ours not only addresses the instance-level retrieval challenge but also mirrors realistic use cases and includes hard negative examples that are semi-automatically collected. \alert{missing link to the following...}

% Recent advances in vision and language models (VLMs) often leverage large-scale training data, which is typically noisy or synthesized due to the challenges of data collection. In contrast, we take a training-free approach that inherently benefits from any future progress in VLMs.
% Our proposed method computes image-to-image and text-to-image similarities separately, then combines them into a single similarity measure, carefully balancing their contributions to prevent one from dominating. We enhance each similarity through simple, efficient, and intuitive operations applied to either the representation or the input space.
% By leveraging the shared image-text space, we obtain an image embedding projection that better represents object instances while remaining invariant to common variations described in text queries. Furthermore, to bridge the gap between the VLMs' original training and the text queries, we employ a contextualization process that enriches the query with multiple plausible words or sentences.
% This approach not only achieves state-of-the-art performance on our newly created dataset but also surpasses existing benchmarks on semantic-level datasets, highlighting its robustness and generalization ability.


% Our contributions are summarized as follows:
% \begin{itemize}
% \item
% \item
% \end{itemize}



%%% imagenet-r from the pic2word paper: We regard the retrieved image as correct if its class and domain match with the query image and domain. Due to the lack of datasets that can evaluate instance-level cross-domain retrieval on diverse samples, we rely on class- and domain-level eval- uation. While not ideal this evaluation can still give us good insight
%%%% fashion-iq - To ensure that the relative captions can describe the fine- grained visual differences between the reference and target image, we leveraged product title information to select sim- ilar images for annotation with relative captions. ALSO: subjective terms: elegant, not always relative.
%%%CIRR:  they lack the sufficient visual complexity to facilitate the study of one of the major challenges in composed image re- trieval, which is the subtle reasoning over what aspects are important and what shall be ignored.. the can- didate images cannot be extensively labeled for each ⟨IR , t⟩ pair, existing datasets contain many false-negatives.
% we collect the mod- ifying text to distinguish the target from a set of similar im- ages (addressing the problem of false-negatives)
%we randomly pick one im- age from the large corpus
%% only 6 images are "hard" negs - no guarantee not to have other false negs....
%%%%% CIRCO -- Furthermore, despite the vi- sual similarity, the difference between images belonging to the same set can possibly be not easily describable with a relative caption and require an absolute description. we start from a single pair of visually similar images and write a relative caption.
% Then, we propose to employ our approach to retrieve the top 100 images according to the query and combine them with the top 50 images most visually similar to the target one. Finally, we select the images that are valid matches for the query.
% CIRR addresses the issue by employing also RecallSubset@K, which considers only the images in the same set of the reference and target ones.



==> tex/method.tex <==
\section{A surprisingly strong baseline}
\label{sec:method}

In the task of \emph{composed image retrieval} (CIR), we are given an image query $q^v \in \cX^v$ and a text query $q^t \in \cX^t$, where $\cX^v$ is the image input space and $\cX^t$ is the text input space. The goal is to retrieve images $x^v$ from a database $X = \{ x_1^v, \dots, x_n^v \} \subset \cX^v$ that are visually relevant to the image query and reflect the modifications specified by the text query. %We are not given any annotation, and whether retrieval is meant to be at class-level or instance-level is only considered at evaluation.
%
Features are extracted using a pre-trained visual encoder $\phi^v: \cX^v \to \real^d$ and text encoder $\phi^t: \cX^t \to \real^d$, \eg CLIP~\cite{clip}, which map image and text queries to a shared embedding space of dimension $d$. 
Image-to-image and image-to-text similarities are computed via dot product of the corresponding features.
% The resulting feature vectors are then combined to produce a single query representation, which is used to compute similarity scores against image embeddings in the database.


% We consider the \emph{composite image retrieval} (CIR) task. Given an image query $q^v$ and a text query $q^t$, the goal is to retrieve the most relevant images $x^v$ from an image database. To solve this task, it is common (\textcolor{red}{is this correct}) to extract features from the queries using pre-trained multimodal encoders $\phi_i$ and $\phi_t$ (\eg CLIP), which map the image and the text into a shared embedding space $\real^d$. The resulting feature vectors are then combined to produce a single query representation, which is used to compute similarity scores against image embeddings in the database.

% Our method assumes that \emph{each modality provides a semantically coherent, complementary path} towards the retrieval goal. This makes the retrieval task analogous to performing a logical “AND” over the two modalities: we seek results that are simultaneously relevant to both the image and the text. This assumption holds well for standard composite tasks (e.g., this image and the concept ``winter”), but may not apply in tasks where one modality dominates (e.g., purely textual transformations) or where the text query is highly entangled with image content (e.g., CIRCO-like datasets). We revisit this in the limitations.

The proposed training-free method, called \ours, is based on the assumption that both modalities in the composed retrieval query encode
% meaningful, semantically coherent, and
complementary information that jointly contribute to the retrieval objective. This makes the composed retrieval task analogous to performing a logical conjunction over the two modalities: we seek results that are simultaneously relevant to both the image and the text \footnote{While this assumption holds well for standard composite tasks (\eg this image and the concept ``winter”), it may not apply in tasks where one modality dominates (\eg purely textual transformations) or where the text query is highly entangled with image content (\eg CIRR-like datasets). In such cases, the benefits of the proposed 
% projection and fusion 
mechanisms may diminish.}.

%--------------------------------------------------------------------
\begin{figure}
\vspace{-10pt}
    \centering
    \includegraphics[width=.97\linewidth]{fig/cir_methodology.pdf}
    %\caption{\emph{Overview of our training-free composed image retrieval \ours method}. Given a query image and text, we apply mean subtraction and semantic projection (guided by corpora $C+$ and $C-$) to filter irrelevant dimensions. The text query is contextualized using caption-like prompts. Both modalities are scored against database items with min-based normalization, then fused via a multiplicative “AND” operation regularized by a Harris-like criterion to retrieve jointly relevant results.}
    \caption{\emph{Overview of our training-free composed image retrieval method \ours.} Given a query image and text, we apply centering and semantic projection, guided by corpora $C+$ and $C-$, to suppress irrelevant dimensions. The text is contextualized using caption-like prompts. Both modalities are scored against the database with min-based normalization and fused via a multiplicative ``AND'' operation regularized by a Harris-like criterion to retrieve jointly relevant results.}
    \label{fig:methodology}
    \vspace{-12pt}
\end{figure}
%--------------------------------------------------------------------

% Our method assumes that both image and text components of a query provide semantically distinct and complementary information. This allows us to interpret similarity multiplication as a logical conjunction operator. However, in tasks where one modality dominates, \eg text-only edits, or where the text query is highly entangled with image content, \eg CIRCO dataset captions, this assumption may not hold. In such cases, the benefits of our projection and fusion mechanism may diminish.


%%
% Even though multimodal models such as CLIP provide aligned representations across textual and visual modalities, these embeddings often encode modality-specific, irrelevant, and spurious features in practice. Visual embeddings can be entangled with background elements, image composition, or dataset-specific styles, while text embeddings may reflect lexical biases or corpus-level drift.
%
Following the aforementioned assumption, we compute the similarity per modality and then combine them.
We improve the representation per modality by removing 
% Under this assumption, it is crucial that the representations from each modality reflect clean and content-relevant 
% semantics, 
% information, as any 
modality-specific noise and spurious correlations that can interfere with their effective combination. 
% While multimodal models such as CLIP provide aligned representations across visual and textual modalities, 
% The features often contain modality-specific noise and spurious correlations. 
In practice, visual features may be entangled with background clutter, image composition, or dataset-specific styles, whereas textual features can reflect lexical biases or corpus-level drift. 
% Such factors can hinder the retrieval of \alert{semantically aligned} results when queries span both modalities.
%
\autoref{fig:methodology} presents a high-level overview of \ours, which  
consists of a sequence of conceptually simple yet effective steps that progressively filter out the aforementioned noise and modality-specific artifacts from the image and text features.
% By isolating semantically meaningful directions within the shared embedding space, \ours facilitates more accurate and reliable similarity computations for composite image retrieval.


% In Figure~\ref{fig:methodology} we illustrate the high level overview of \ours. \ours consists of a sequence of conceptually simple steps that progressively filter out the aforementioned irrelevant factors and modality-specific noise from the image and text features. By isolating semantically meaningful directions, \ours enables more accurate similarity computations.


% and significantly improves retrieval performance.

% The following subsections describe each step of \ours in detail.

% \ours follows the next steps (which are then described in detail):

% \begin{enumerate}
%     \item Mean subtraction to remove modality-specific biases.
%     \item Contextualization of text queries for more robust textual features.
%     \item Projection to a semantic subspace which strips the image style.
%     \item Query expansion to increase the robustness in the image query.
%     \item Score normalization to balance the two modalities and harris criterion robust fusion.
% \end{enumerate}

%--------------------------------------------------------------------

\textbf{Centering for bias removal.}
% As the first step, we aim to 
We remove modality-specific biases by subtracting mean features. These means typically capture low-level regularities unique to each modality: the average image feature reflects general 
% ``imageness,'' 
visual patterns,
while the average text feature captures 
% generic 
% ``textness.'' 
common linguistic patterns.
Subtracting them helps isolate semantic content from distributional bias.
%
In particular, after extracting the image
% query 
features $\vq^v = \phi^v(q^v) \in \real^d$ and text
% query
features $\vq^t = \phi^t(q^t) \in \real^d$, 
also from the database images, 
we subtract  a precomputed image feature mean $\vmu^v \in \real^d$, 
% which filters out common visual patterns unrelated to semantics, 
and a text feature mean $\vmu^t \in \real^d$, respectively.
% which removes corpus-level linguistic drift. 
The centered features are
\begin{equation}
	\bar{\vq}^v = \vq^v - \vmu^v = \phi^v(q^v) - \vmu^v
	\quad \text{and} \quad
	\bar{\vq}^t = \vq^t - \vmu^t = \phi^t(q^t) - \vmu^t.
\end{equation}
To ensure scalability and generalization, we compute $\vmu^v$ using a large external dataset $X^v$, \eg LAION~\cite{laion}. Similarly, we calculate the text mean $\vmu^t$ on a 
% manually defined 
predefined textual corpus which contains content-relevant concepts (see next step).
% To ensure scalability and generalization, we compute $\vmu^v$ using a large external dataset $X^v$, \eg LAION. While dataset-specific means can further boost performance, they assume access to a thematically consistent and curated corpus, which is often unrealistic in open-world retrieval settings. \textcolor{red}{Similarly, we calculate the text mean $\vmu^t$ on a manually defined textual corpus $X^t$, which contains content-relevant concepts:}

% \begin{equation}
% 	\vmu^v = \frac{1}{\card{X^v}} \sum_{x \in X^v} \phi^v(x)
% 	\quad \text{and} \quad
% 	\vmu^t = \frac{1}{\card{X^t}} \sum_{x \in X^t} \phi^t(x).
% \end{equation}

%--------------------------------------------------------------------

\textbf{Projection onto semantic subspace.}
%Next, we want to
% The next step 
% is designed to 
% We aim to suppress 
% semantically irrelevant 
% style, context, or domain related 
% information from the image features while retaining information related to the main 
% subject 
% object
% of the image. 
We aim to transform the image features to retain information related to the main objects, while suppressing information related to image styles, object domains, or background setting, \ie that correspond to text query modifications of common use cases.
% In particular, the centered image features are
This is achieved by 
projecting into a lower-dimensional subspace derived from text CLIP features.
%
To construct this projection, we use two textual corpora: $C_+$, a \emph{object corpus} containing object-oriented terms (\eg ``building'', or ``dog''), and $C_-$, a \emph{stylistic corpus} containing terms related to style, viewing conditions or contextual setting (\eg ``cartoon'', ``aerial view'', or  ``in a cloudy day''). 
% These corpora define contrastive semantic directions: $C_+$ highlights directions we aim to retain, while $C_-$ identifies directions to suppress. 
% The rationale is to emphasize object-specific semantic directions while attenuating style-related variations. 
Inspired by~\cite{oldfield2023parts}, we compute a weighted contrastive covariance matrix as follows :
%
% To construct this projection, we apply PCA to two manually defined textual corpora: $C_+$, a \emph{subject-oriented corpus} containing content-relevant concepts (\eg ``building,'' ``dog''), and $C_-$, a \emph{stylistic corpus} containing distractors related to style, appearance, or background (\eg ``origami,'' ``sunset''). These corpora define contrastive semantic directions: $C_+$ highlights directions we aim to retain, while $C_-$ identifies directions to suppress. The rationale is to emphasize subject-specific semantic directions while attenuating style-driven variations. We now compute a weighted contrastive covariance matrix as follows:
\begin{equation}
	\vC = (1 - \alpha) \vC_+ - \alpha \vC_-,
	\quad \text{where} \quad
	\vC_\pm = \frac{1}{|C_\pm|} \sum_{x \in C_\pm}
		(\phi^t(x) - \vmu^t) (\phi^t(x) - \vmu^t)^\top
\end{equation}
% \textcolor{red}{say about alpha}
% and $\alpha$ is an empirically determined hyperparameter. We extract the top-$k$ eigenvectors of $\vC \in \real^{d \times d}$ to form a projection matrix $\vP \in \real^{d \times k}$. 
% The eigenvectors are directions that have large variance in $\vC_+$ and small in $\vC_-$.
% The rationale is to emphasize object-specific directions while attenuating style-related variations. 
% We then project the centered image features $\bar{\vx}^v = \phi(x^v) - \vmu^v \in \real^d$, either query or database, as $\vP^\top \bar{\vx}^v \in \real^k$.
% %
% Note that the corpora $C_+$ and $C_-$ need not match the domain of the retrieval database. Even generic corpora for $C_+$, \eg class names from ImageNet, yield performance improvements, because the directions they capture are semantically rich and broadly transferable. 
and $\alpha$ is an empirically determined hyperparameter. We extract the top-$k$ eigenvectors of $\vC \in \real^{d \times d}$ to form a projection matrix $\vP \in \real^{d \times k}$. 
The eigenvectors capture directions with high variance in $\vC_+$ and small in $\vC_-$,
emphasizing object-specific cues while suppressing style-related variation.
We then project the centered image features $\bar{\vx}^v = \phi(x^v) - \vmu^v \in \real^d$, either query or database, as $\vP^\top \bar{\vx}^v \in \real^k$.
%
Note that the corpora $C_+$ and $C_-$ need not match the domain of the retrieval database. Even generic corpora for $C_+$, \eg class names from ImageNet-1K~\cite{dsl+09}, yield performance improvements, as the captured directions are semantically rich and broadly transferable.

% \textcolor{red}{By describing the content-relevant part of the image as a linear combination of basis vectors obtained from such corpora, we are not only limited to class-based retrieval, but may also extend to instance-level retrieval.}

%--------------------------------------------------------------------

%\paragraph{Efficient computation}
%
%To avoid costly reprojection of all dataset embeddings, we leverage an efficient formulation for computing similarities the similarity $s^v$ between the centered query image embedding $\bar{\vq}^v \in \real^d$ and database image embedding $\bar{\vx}^v \in \real^d$ for retrieval:
%\begin{equation}
%	s^v = \inner{\vP^\top \bar{\vx}^v, \vP^\top \bar{\vq}^v}
%		= (\bar{\vx}^v)^\top \vP \vP^\top \bar{\vq}^v
%		= \inner{\bar{\vx}^v, \vP \vP^\top \bar{\vq}^v}.
%\end{equation}
%Thus, we only need to project query embeddings, avoiding any additional computation on the dataset embeddings at retrieval time.

% and obtain the top $k$ (< $d$) eigenvectors, forming a projection matrix $\vP_r$ that reduces dimensionality from $d$ to $k$. The projected image features are then calculated as
% %\begin{equation}
% $\vP_r^\top (\phi(\vI) - \vmu_{img}) = \vP_r^\top \bar{\vx} $.
% %\end{equation}

% We note that the text corpora we used do not need not match the retrieval dataset's domain. Even general corpora (\eg ImageNet class names) yield performance improvements, because the directions they capture are semantically rich and broadly transferable. By describing the content-relevant part of the image as a linear combination of the basis function of such corpora, we cannot only perform class-based retrieval~\cite{}, but also extend to instance-level retrieval.

% Notably, to avoid having to project all the image embeddings in the dataset (which would be a significant computation step), we can avoid this wit the following formulation by calculating the retrieval simalarity between the centered query embedding $\bar{\vx}_q$ and the centered embedding of a sample from the dataset $\bar{\vx}_i$ by computing the following inner product:
% \begin{equation}
% s_i = \langle \vP_r^\top \bar{\vx}_i,  \vP_r^\top \bar{\vx}_q \rangle =\bar{\vx}_i^\top \vP_r\vP_r^\top \bar{\vx}_q = \bar{\vx}_i^\top (\vP \bar{\vx}_q) ,
% \quad \text{where} \quad \vP = \vP_r \vP_r^\top
% \end{equation}
% Note that the projection matrix $\vP$ (which does not reduce dimensionality anymore), can be only applied to the query embeddings, avoiding any extra operation on the dataset side.

%--------------------------------------------------------------------

\textbf{Image query expansion.}
In the literature, image retrieval performance, recall in particular, has been shown to be significantly improved by query expansion~\cite{cps+07,grb20}. The proposed method benefits from applying the \emph{optional} step of query expansion 
using the image query.
% in the visual part of the similarity measure. 
Following~\cite{grb20}, the original feature of the image query is enhanced by a weighted combination of the top-ranked database features that it retrieves. 
The weights are an increasing function of the corresponding similarities.
% with the original query. 
%All operations are evaluated with centered representations and after projection onto the semantic subspace.

%To handle high intra-class variation or diverse viewpoints (\eg in instance-level retrieval), we refine the initial projected query image  $\vP\vP^\top \bar{\vq}^v \in \real^d$ by fetching its top-$k$ nearest neighbors in the centered database. 
%The expanded query $\tilde{\vq}^v \in \real^d$ is computed via a soft attention-weighted mean over these top-$K$ features and then reprojected into the semantic subspace.
%Since the projected space is used, this step captures semantically consistent variations over the 
 %depicted subjects, ignoring irrelevant background or stylistic elements. 
%This captures semantically consistent appearance variations, focusing on the subject rather than noise - since we use the projected space, and boosts robustness.


%The resulting embedding is again projected into the semantic subspace. This step improves robustness by incorporating appearance variation that is semantically consistent with the original query, especially given the fact that the neighboring samples are calculated on the projected space and thus focusing only on the subject and not potential noise.

% \subsection{Query expansion}
% \textcolor{red}{can be written in two lines - suppl. for details}

% In tasks with high intra-class variation or viewpoint diversity, \eg instance-level retrieval, it can be beneficial to refine the query using the database. We define a simple but effective form of \emph{query expansion}. Given the initial projected query image $\vP\vP^\top \bar{\vq}^v \in \real^d$, we compute its top-$k$ nearest neighbors $\{ z_1^v, \dots, z_k^v \} \subset X$ in the database $X$. Their centered features $\bar{\vz}_i^v = \phi^v(z_i^v) - \vmu^v \in \real^d$ are aggregated into an expanded query $\tilde{\vq}^v \in \real^d$ via a soft attention-weighted mean:
% \begin{equation}
% 	\tilde{\vq}^v = \sum_{i=1}^k w_i \bar{\vz}_i^v,
% 	\quad \text{where} \quad
% 	w_i = \frac{\exp(\beta \inner{\bar{\vz}_i^v, \vP\vP^\top \bar{\vq}^v})}
% 		{\sum_{j=1}^k \exp(\beta \inner{\bar{\vz}_k^v, \vP\vP^\top \bar{\vq}^v})}.
% \end{equation}
% The resulting embedding is again projected into the semantic subspace. This step improves robustness by incorporating appearance variation that is semantically consistent with the original query, especially given the fact that the neighboring samples are calculated on the projected space and thus focusing only on the subject and not potential noise.

%--------------------------------------------------------------------

\textbf{Contextualization of text queries.}
CLIP is trained primarily on natural language captions and full sentences.
% , rather than isolated 
% words or sentence parts.
% category names or sentence parts. 
As a result, using single-word text queries (\eg \texttt{``sculpture''}) or sentence parts (\eg \texttt{``during sunset''}) constitute out-of-distribution input and may produce text
% such ``partial'' 
features that are not well-aligned with image features. 
To address this, we introduce a \emph{contextualization} step that enriches 
% sparse
such 
textual queries with additional terms.
% noun phrases.
%
Let $q^t$ be a raw text query (\eg \texttt{``sculpture''}).
% and let $C_+$ be a fixed \emph{context vocabulary} (\eg a set of common nouns like ``dog'', ``train'', etc.). 
We generate multiple caption-like queries by combining $q^t$ with elements from the subject corpus $C_+$. We add a random set of terms 
before (\eg \texttt{``dog during the sunset''}) and after (\eg \texttt{``sculpture dog''}) the text query. These composed phrases are embedded using CLIP's text encoder, centered, and averaged.
This operation yields a more robust
% subject-aware
textual feature that better reflects how CLIP interprets concepts in natural language (\eg \texttt{``[something] during the sunset''}). 

%This operation yields a more robust, subject-aware textual feature that better reflects how CLIP interprets concepts in natural language (\eg ``[something] during the sunset''). 
%This step is particularly effective when the raw query consists of abstract categories or adjectives (\eg ``ancient'', ``wooden'', ``patterned'').

%--------------------------------------------------------------------

\paragraph{Score normalization and fusion.}

% The final step is to combine similarities from the image and text modalities and rank database items accordingly. Following the aforementioned definitions, we calculate the similaries as follows:
% %Let $\hat{\phi}(D)$ be the (projected) embedding of a database item. We compute:

% \begin{equation}
% s^{\text{img}}_i = \langle \vP^\top \tilde{\vx}_q, \bar{\vx}_i \rangle, \quad s^{\text{text}}_i = \langle \bar{\vx}_t, \bar{\vx}_i \rangle.
% \end{equation}
% where $\bar{\vx}_t = \phi_c(q^t) - \vmu^t$ is the centered contextualized version of the text query $q^t$.

% % Our method assumes that \emph{each modality provides a semantically coherent, complementary path} towards the retrieval goal. This makes the retrieval task analogous to performing a logical “AND” over the two modalities: we seek results that are simultaneously relevant to both the image and the text. This assumption holds well for standard composite tasks (\eg this image and the concept ``winter”), but may not apply in tasks where one modality dominates (\eg purely textual transformations) or where the text query is highly entangled with image content (\eg CIRCO-like datasets). We revisit this in the limitations.

% In order to combine the similarities we follow a logical ``AND" approach over the two modalities in order to combine the similarities, by calculating the proudct of the two similarities  $s_i = s^{\text{img}}_i \cdot s^{\text{text}}_i.$

% % Moreover, zero similarity in one modality could diminish the results, but in a multiplication paradigm this zero "neutral" similarity could better correspond to 1, the neutral element of multiplication.

% % Following the ``AND'' rationale for combining modalities, the composite similarity for a database item $i$ is computed as:
% % \begin{equation}
% % s_i = s^{\text{img}}_i \cdot s^{\text{text}}_i.
% % \end{equation}

% This multiplicative fusion emphasizes candidates that are jointly relevant to both the image and text queries. However, the raw similarity scores $s^{\text{img}}$ and $s^{\text{text}}$ may lie in different numerical ranges due to modality differences, centering, and the image-space projection. This imbalance can lead to one modality dominating the other during fusion.

% Additionally, a score of zero in one modality (often the result of mean subtraction or semantic irrelevance) would collapse the product to zero, even if the other modality provides a strong signal. Under this paradigm, it is more appropriate to treat a zero similarity as a ``neutral'' signal—closer in behavior to 1, the multiplicative identity.

% To mitigate these issues, we introduce a normalization step that treats zero similarity as a neutral signal, followed by a regularized fusion mechanism inspired by the Harris corner detector to balance contributions from both modalities.

% The final step is to combine similarities from the image and text modalities to rank the database items. Given the projected image query embedding $\tilde{\vq}^v \in \real^d$ and the contextualized centered text query embedding $\bar{\vq}^t = \phi^t(q^t) - \vmu^t \in \real^d$, we compute similarities to the centered embedding $\bar{\vx}^v \in \real^d$ of a database image $x^v \in X$ as:
% \begin{equation}
% 	s^v = \inner{\bar{\vx}^v, \vP\vP^\top \tilde{\vq}^v}
% 	\quad \text{and} \quad
% 	s^t = \inner{\bar{\vx}^v, \bar{\vq}^t}.
% \end{equation}
% To reflect the complementary nature of the modalities, we fuse the two scores by multiplication: $s = s^v s^t$. This formulation emphasizes database items that are jointly relevant to both the visual and textual cues. However, due to modality imbalance and differences in representation ranges, one modality can disproportionately dominate the final score. Additionally, zero similarity in one modality—often caused by mean subtraction or irrelevant content—can collapse the product to zero, despite strong relevance in the other modality.

The final step is to combine similarities from the two modalities to rank the database items. Given the centered image query embedding $\bar{\vq}^v \in \real^d$ and the contextualized centered text query (either original, or expanded) embedding $\bar{\vq}^t \in \real^d$, we compute similarities to the centered embedding $\bar{\vx}^v \in \real^d$ of a database image $x^v \in X$ as:
\begin{equation} \label{eqn:score}
	s^v = \inner{\vP^\top \bar{\vx}^v, \vP^\top \bar{\vq}^v}
	\quad \text{and} \quad
	s^t = \inner{\bar{\vx}^v, \bar{\vq}^t}.
\end{equation}
To reflect the complementary nature of the modalities, we fuse the two scores by multiplication: $s = s^v s^t$. 
%This formulation emphasizes database items that are jointly relevant to both the visual and textual cues. 
However, due to modality imbalance and differences in representation ranges, one modality can disproportionately dominate the final score. 
%Additionally, zero similarity in one modality—often denoting irrelevant content—can collapse the product to zero, despite strong relevance in the other modality.

%--------------------------------------------------------------------

%\paragraph{Min-based normalization}

% To mitigate these issues we introduce a simple normalization step that rescales each similarity score based on its empirical lower bound:
% \begin{equation}
% \tilde{s} = \frac{s - s_{\min}}{|s_{\min}|}, \quad \text{where } s_{\min} < 0.
% \end{equation}
% This maps $s = s_{\min}$ to 0 and $s = 0$ to 1, treating zero similarity as the neutral value. Such normalization preserves meaningful contrast and ensures that modality scores are better balanced before fusion.

% We apply this function to both $s^{\text{img}}$ and $s^{\text{text}}$ similarities using predefined statistical values for $s^{\text{img}}_{\min}$ and $s^{\text{text}}_{\min}$ that take into account the CLIP backbone, as well as the projection. For more details see suppl. material.

% To mitigate these issues, we apply a simple normalization step based on the empirical minimum of similarity scores:
% \begin{equation}
% 	\tilde{s} = \frac{s - s_{\min}}{|s_{\min}|},
% 	\quad \text{where} \quad s_{\min} < 0.
% \end{equation}
% \textcolor{red}{(What if $s_{\min} \ge 0$?)}
% This maps $s = s_{\min}$ to 0 and $s = 0$ to 1, treating zero similarity as neutral. We apply this to both $s^v$ and $s^t$ using predefined statistics for $s^v_{\min}$ and $s^t_{\min}$, estimated on an external dataset. See supplementary material for details.

\textit{Min-based normalization.}
%To treat zero similarity as neutral and 
To mitigate range imbalances, an affine re-scaling of the similarities $s$ in each modality is performed. The empirical minimum $s_{\min}<0$ of the dot product in (\ref{eqn:score}) is used, so that $s_{\min}$ is mapped to $0$ and $0$ is mapped to $1$:
%\[
%\tilde{s} \;=\;\frac{s - s_{\min}}{|s_{\min}|}\,
%\]
\[
\tilde{s} \;=\; (s - s_{\min}) / |s_{\min}|.
\]
We apply this to both $s^v$ and $s^t$ using predefined statistics for $s^v_{\min}$ and $s^t_{\min}$, estimated on an external dataset.
%See~\autoref{sec:suppl_method} for more details.
%We precompute $s^v_{\min}$ and $s^t_{\min}$ on an external dataset (see supplementary material).

%--------------------------------------------------------------------

\textit{Fused similarity with Harris criterion.}
Finally, we fuse the normalized scores using multiplication and a regularizer inspired by the Harris corner detector. The final score is:
\[
	\tilde{s}^f = \tilde{s}^v \tilde{s}^t -
	\lambda (\tilde{s}^v + \tilde{s}^t)^2.
\]
The first term rewards items that are jointly relevant to both modalities. The second term penalizes items where only one modality is highly activated, thereby suppressing false positives from unbalanced queries. The scalar $\lambda$ controls the trade-off and is fixed across all experiments.
%--------------------------------------------------------------------

\textbf{Computational complexity.}
%One of the key 
The strengths of our approach stem from its simplicity and efficiency. The entire pipeline is (deep-network) training-free and is composed of operations that scale linearly or sub-linearly with the dataset size, since similarity computation over the dataset items is a simple inner product and can be efficiently handled by existing libraries, \eg FAISS~\cite{jdh17}. 
%
The proposed similarity computation efficiently operates over a stored database of original CLIP representations. The similarity $s^v$ is efficiently computed as follows
%
%To avoid costly reprojection of all dataset embeddings, we leverage an efficient formulation for computing similarities the similarity $s^v$ between the centered query image embedding $\bar{\vq}^v \in \real^d$ and database image embedding $\bar{\vx}^v \in \real^d$ for retrieval:
%
% \begin{eqnarray*}
%  s^v & = & %\inner{\vP^\top \bar{\vx}^v, \vP^\top \bar{\vq}^v} =
%  \inner{\vP^\top ({\vx}^v - \mu^v), \vP^\top ({\vq}^v - \mu^v)}
% 		= ({\vx}^v - \mu^v)^\top \vP \vP^\top ({\vq}^v - \mu^v) \\
% 		& = & \inner{\vx^v, \vP \vP^\top ({\vq}^v - \mu^v)} -  \inner {\mu^v, \vP \vP^\top ({\vq}^v - \mu^v)} \mbox{,}
% \end{eqnarray*}
\[
 s^v  =  %\inner{\vP^\top \bar{\vx}^v, \vP^\top \bar{\vq}^v} =
 \inner{\vP^\top ({\vx}^v - \vmu^v), \vP^\top ({\vq}^v - \vmu^v)}
		= \inner{\vx^v, \vP \vP^\top ({\vq}^v - \vmu^v)} -  \inner {\vmu^v, \vP \vP^\top ({\vq}^v - \vmu^v)} \mbox{,}
\]
where the first term is a dot-product computed over the unaltered database features and the second term is a query dependent constant. Thus, all computation related to centering and projection can be computed on-the-fly on the query side. This is valuable, since the mean and the projection matrix can be alternated (\eg with specific knowledge of the domain) without touching the stored index.
This makes our method particularly well-suited for large-scale deployments, requiring no adaptation, no fine-tuning, and no backpropagation. See the supplementary material for more technical details.

%The projection matrix, the means required for centering and the $s_{\min}$ statistics are all precomputed, while centering of the dataset can also be computed offline.  Query expansion adds negligible complexity as it only involves top-$k$ retrieval and weighted averaging.

%One of the key strengths of our approach lies in its efficiency and simplicity. The entire pipeline is training-free and composed of operations that scale linearly or sub-linearly with the dataset size: 



% \begin{itemize}
%     \item \textbf{Centering and projection} are applied once per embedding and require matrix-vector multiplications of complexity $O(dk)$, where $k \ll d$.
%     \item \textbf{Similarity computation} is done via matrix-vector  multiplication of complexity $O(nk)$ for $n$ database items, which is efficiently handled by existing libraries, \eg FAISS.
%     \item \textbf{Query expansion} adds negligible complexity as it only involves top-$k$ retrieval and weighted averaging.
%     \item \textbf{No normalization per query or feature is required at test time}. All embeddings are precomputed; query evaluation consists of fast dot products and scalar operations.
% \end{itemize}


% \subsection{Limitations}

% Our method assumes that both image and text components of a query provide semantically distinct and complementary information. This allows us to interpret similarity multiplication as a logical conjunction operator. However, in tasks where one modality dominates, \eg text-only edits, or where the text query is highly entangled with image content, \eg CIRCO dataset captions, this assumption may not hold. In such cases, the benefits of our projection and fusion mechanism may diminish.


==> tex/method_old.tex <==
\section{Method}
\label{sec:method}


Our approach is a training-free retrieval framework that enhances composite queries in the CLIP embedding space. The core idea is to remove irrelevant or noisy variation from image features and emphasize semantically meaningful directions using lightweight, deterministic transformations. This is done through a set of empirically validated, conceptually simple steps that we consider as a form of \emph{best practices} for zero-shot retrieval. These include modality-specific mean subtraction, projection into a semantic subspace derived from text embeddings, textual contextualization, query expansion, and principled score normalization and fusion.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{fig/cir_methodology.pdf}
    \caption{\emph{Overview of our training-free composed image retrieval \ours method}. Given a query image and text, we apply mean subtraction and semantic projection (guided by corpora $\mathcal{C}+$ and $\mathcal{C}-$) to filter irrelevant dimensions. The text query is contextualized using caption-like prompts. Both modalities are scored against database items with min-based normalization, then fused via a multiplicative “AND” operation regularized by a Harris-like criterion to retrieve jointly relevant results.}
    \label{fig:methodology}
\end{figure}

\subsection{Motivation}

We begin with the assumption that a composite retrieval query consists of two distinct semantic paths—typically, an image and a textual description—each encoding meaningful content. CLIP provides aligned representations across these modalities, enabling retrieval via similarity comparison in a shared embedding space. However, in practice, CLIP embeddings often encode both content and spurious dimensions: visual embeddings are entangled with background, composition, and dataset-specific style; text embeddings reflect lexical biases or corpus-level drift.

Our method assumes that \emph{each modality provides a semantically coherent, complementary path} towards the retrieval goal. This makes the retrieval task analogous to performing a logical “AND” over the two modalities: we seek results that are simultaneously relevant to both the image and the text. This assumption holds well for standard composite tasks (e.g., this image and the concept ``winter”), but may not apply in tasks where one modality dominates (e.g., purely textual transformations) or where the text query is highly entangled with image content (e.g., CIRCO-like datasets). We revisit this in the limitations.




\subsection{Definitions}

We have a dataset of images $I_D$ and image and text queries $I_q$ and $I_t$. 
In this work we rely on corpora to find a proper semantic projection space.
We have the subject-oriented corpus $C_{+}$ and the stylistic-oriented corpus $C_{-}$. Both have textual descriptions and are pre-defined by the user.
We extract the embeddings of all these data using multi-modal feature extractors $\phi_i(\cdot)$ and $\phi_t(\cdot)$, one for each modality, like CLIP.  


Let $I_D$ be the image database and $(I_q, T_q)$ the image and text components of a retrieval query. Features are extracted using pretrained multi-modal encoders $\phi_i(\cdot)$ and $\phi_t(\cdot)$ (e.g., CLIP), mapping images and text into a shared embedding space $\mathbb{R}^d$.
\[
\phi_i(I) \in \mathbb{R}^d, \quad \phi_t(T) \in \mathbb{R}^d.
\]

\textcolor{red}{filby -> its better to define what exactly we want the projection to do before describing it}


To construct a semantic projection space, we use two user-defined textual corpora: 
$\bullet$ $\mathcal{C}_{+}$: a \textit{subject-oriented corpus} capturing content-relevant concepts (e.g., ``building'', ``dog'').
$\bullet$ $\mathcal{C}_{-}$: a \textit{stylistic corpus} capturing distractors such as appearance, lighting, or background style (e.g., ``origami'', ``sunset'').
These corpora guide the projection step: $\mathcal{C}_{+}$ acts as a set of semantic \emph{attractors}, while $\mathcal{C}_{-}$ defines directions to suppress.


\subsection{Mean Subtraction for Bias Removal}

The first step removes modality-specific biases by subtracting mean embeddings, which typically capture low-level regularities that differ between the two modalities. The mean of image CLIP embeddings often reflects “imageness”, while the mean of textual embeddings captures generic “textness”. Removing these helps isolate semantic content from distributional priors.

%Let $\phi(I), \phi(T) \in \mathbb{R}^d$ be image and text embeddings. 
Specifically, we subtract the mean of image embeddings $\mathbf{\mu}_{\text{vis}}$, removing common visual pattern irrelevant to the semantic information,
and the mean of the text corpus $\mathbf{\mu}_{\text{text}}$ (here we use the mean of $\mathcal{C}_{+}$ embeddings), removing common linguistic drift.

While dataset-specific visual means can boost retrieval performance, they assume access to a curated and thematically consistent dataset—an unrealistic assumption in many real-world scenarios. For scalability and generalization, we instead favor using a generic visual mean, estimated from external datasets (e.g., LAION). This allows our method to operate effectively across diverse and unstructured domains without retraining or adaptation.

\subsection{Contextualization of Text Queries}

CLIP is trained primarily on natural language captions and full sentences, rather than isolated category names or sentence parts. As a result, using single-word prompts (e.g., ``sculpture'') or part-sentences (e.g., ``during sunset") may produce such ``partial" representations that are not well-aligned with image embeddings. To address this, we introduce a \emph{contextualization} step that enriches sparse textual queries with compatible noun phrases.

Let $T_q \in \mathbb{R}^d$ be the raw text query (e.g., ``sculpture'') and let $\mathcal{C}_{+}$ be a fixed context vocabulary (e.g., a set of common nouns like ``dog'', ``train'', etc.). For each query, we generate multiple caption-like prompts by combining it with elements from $\mathcal{C}$. We add a random set of nouns before ("dog + during the sunset") and after ("sculpture + dog") the text query. These composed phrases are embedded using CLIP’s text encoder and averaged. 

This operation yields a more robust, subject-aware textual feature that better reflects how CLIP interprets concepts in natural language (e.g., ``[something] during the sunset"). This step is particularly effective when the raw query consists of abstract categories or adjectives (e.g., ``ancient'', ``wooden'', ``patterned'').

\paragraph{Practical Efficiency.} This step requires only one forward pass through CLIP’s text encoder for a fixed set of composed prompts and can be cached per corpus. It adds no inference cost during retrieval.

\subsection{Projection onto Semantic Subspace}

% On the core of this proposed approach, we aim to assist the image query by stripping out any semantically irrelevant information from the image modality. In other words, we want the image embeddings to be projected into a sub-space where we have information only for the ``main character" of the image, the subject. 

The goal of the projection step is to suppress semantically irrelevant information from image features, thereby isolating features related to the image's main subject.


To isolate semantically meaningful directions, we project the centered image features into a lower-dimensional subspace derived from text CLIP embeddings. This projection acts as a filter, suppressing components that do not align with concepts present in the textual domain.

Specifically, we construct the semantic subspace by applying PCA to a corpus of text embeddings $\mathcal{C}_+$. Additionally, we introduce a negative corpus $\mathcal{C}_-$ consisting of distractor concepts (e.g., stylistic terms). From these, we compute their contrastive covariance:

\[
\mathbf{C} = (1 - \alpha) \mathbf{C}_{+} - \alpha \mathbf{C}_{-}, \quad \text{where} \quad \mathbf{C}_{\pm} = \frac{1}{|\mathcal{C}_\pm|} \sum_{x \in \mathcal{C}_\pm} (x - \mathbf{\mu}_{text})(x - \mathbf{\mu}_{text})^\top,
\]

and obtain the top $k$ (< $d$) eigenvectors, forming a projection matrix $\mathbf{P}_r$ that reduces dimensionality from $d$ to $k$. The projected image features are then calculated as 
%\[
$\mathbf{P}_r^\top (\phi(\mathbf{I}) - \mathbf{\mu}_{img}) = \mathbf{P}_r^\top \mathbf{\bar{x}} $.
%\]

This projection captures content-relevant variations and discards common or irrelevant ones. Notably, the text corpus used to compute $\mathbf{P}_r$ need not match the retrieval dataset's domain. Even general corpora (e.g., ImageNet class names) yield performance improvements, because the directions they capture are semantically rich and broadly transferable. By describing the content-relevant part of the image as a linear combination of the basis function of such corpora, we cannot only perform class-based retrieval~\cite{}, but also extend to instance-level retrieval. 

An important implementation aspect can be derived by exploring the similarity score of the image modality. According to our formulation, we can calculate the retrieval similarity between the centered query embedding $\mathbf{\bar{x}}_q$ and the centered embedding of a sample from the dataset $\mathbf{\bar{x}}_i$ by computing the following inner product:
\[
s_i = \langle \mathbf{P}_r^\top \mathbf{\bar{x}}_i,  \mathbf{P}_r^\top \mathbf{\bar{x}}_q \rangle =\mathbf{\bar{x}}_i^\top \mathbf{P}_r\mathbf{P}_r^\top \mathbf{\bar{x}}_q = \mathbf{\bar{x}}_i^\top (\mathbf{P} \mathbf{\bar{x}}_q) ,
\quad \text{where} \quad \mathbf{P} = \mathbf{P}_r \mathbf{P}_r^\top
\]
Note that the projection matrix $\mathbf{P}$ (which does not reduce dimensionality anymore), can be only applied to the query embeddings, avoiding any extra operation on the dataset side.  
\subsection{Query Expansion}

In tasks with high intra-class variation or viewpoint diversity (e.g., instance-level landmark retrieval), it can be beneficial to refine the query representation using the retrieval database. We implement a simple but effective form of \emph{query expansion}.

Given the initial projected query $\mathbf{P}^\top \mathbf{\bar{x}}_q$, we compute its top-$k$ nearest neighbors in the database. These are aggregated into an expanded query via a soft attention-weighted mean:

\[
\mathbf{\tilde{x}}_q = \sum_{i=1}^k w_i \mathbf{\bar{x}}_i, \quad w_i \propto \exp(\beta \cdot \text{sim}(\mathbf{P}^\top \mathbf{\bar{x}}_q, \mathbf{\bar{x}}_i)).
\]

The resulting embedding is then reprojected into the semantic subspace. This step improves robustness by incorporating appearance variation that is semantically consistent with the original query, especially given the fact that the neighboring samples are calculated on the projected space and thus focusing only on the subject and not potential noise.

\subsection{Score Normalization and Fusion}

The final step is to combine similarities from the image and text modalities and rank database items accordingly. Following the aforementioned definitions, we have:
%Let $\hat{\phi}(D)$ be the (projected) embedding of a database item. We compute:

\[
s^{\text{img}}_i = \langle \mathbf{P}^\top \mathbf{\tilde{x}}_q, \mathbf{\bar{x}}_i \rangle, \quad s^{\text{text}}_i = \langle \mathbf{\bar{x}}_t, \mathbf{\bar{x}}_i \rangle.
\]
where $\mathbf{\bar{x}}_t = \phi_c(T_q) - \mathbf{\mu}_{text}$ is the centered contextualized version of the text query $T_q$.

Moreover, zero similarity in one modality could diminish the results, but in a multiplication paradigm this zero "neutral" similarity could better correspond to 1, the neutral element of multiplication.

Following the ``AND'' rationale for combining modalities, the composite similarity for a database item $i$ is computed as:
\[
s_i = s^{\text{img}}_i \cdot s^{\text{text}}_i.
\]
This multiplicative fusion emphasizes candidates that are jointly relevant to both the image and text queries. However, the raw similarity scores $s^{\text{img}}$ and $s^{\text{text}}$ may lie in different numerical ranges due to modality differences, centering, and the image-space projection. This imbalance can lead to one modality dominating the other during fusion.

Additionally, a score of zero in one modality (often the result of mean subtraction or semantic irrelevance) would collapse the product to zero, even if the other modality provides a strong signal. Under this paradigm, it is more appropriate to treat a zero similarity as a ``neutral'' signal—closer in behavior to 1, the multiplicative identity.

\paragraph{Min-Based Normalization.}

To address these issues, we apply a simple normalization strategy that rescales each similarity score based on its empirical lower bound:
\[
\tilde{s} = \frac{s - s_{\min}}{|s_{\min}|}, \quad \text{where } s_{\min} < 0.
\]
This maps $s = s_{\min}$ to 0 and $s = 0$ to 1, treating zero similarity as the neutral value. Such normalization preserves meaningful contrast and ensures that modality scores are better balanced before fusion. 

We apply this function to both $s^{\text{img}}$ and $s^{\text{text}}$ similarities using predefined statistical values for $s^{\text{img}}_{\min}$ and $s^{\text{text}}_{\min}$ that take into account the CLIP backbone, as well as the projection. For more details see suppl. material.

\textcolor{red}{harris can be one sentence}
\paragraph{Fused Similarity with Harris Criterion.}

We can then fuse the normalized scores using a multiplicative operator and a regularizer inspired by the Harris corner detector. The final score is:

\[
\tilde{s}_i = \tilde{s}^{\text{img}}_i \cdot \tilde{s}^{\text{text}}_i - \lambda \cdot (\tilde{s}^{\text{img}}_i + \tilde{s}^{\text{text}}_i)^2.
\]

The first term rewards items that are jointly relevant to both modalities. The second term penalizes cases where only one modality is highly activated, thereby suppressing false positives from unbalanced queries. The scalar $\lambda$ controls the trade-off and is fixed across all experiments.

\subsection{Computational Complexity and Efficiency}

One of the key strengths of our approach lies in its efficiency and simplicity. The entire pipeline is training-free and composed of operations that scale linearly with the dataset size:

\begin{itemize}
    \item \textbf{Centering and projection} are applied once per embedding and require matrix-vector multiplications of $O(dk)$, where $k \ll d$.
    \item \textbf{Similarity computation} is done via matrix multiplication ($O(nk)$ for $n$ database items), which is efficiently handled by existing libraries (e.g., FAISS).
    \item \textbf{Query expansion} adds negligible cost as it only involves top-$k$ retrieval and weighted averaging.
    \item \textbf{No normalization per query or feature is required at test time}. All embeddings are precomputed; query evaluation consists of fast dot products and scalar operations.
\end{itemize}

This makes our method particularly well-suited for large-scale deployments, requiring no adaptation, no fine-tuning, and no backpropagation.

\subsection{Limitations}

Our method assumes that both image and text components of a query provide semantically distinct and complementary information. This allows us to interpret fusion as a logical “AND” operator. However, in tasks where one modality dominates (e.g., text-only edits) or where the text query is highly entangled with image content (e.g., CIRCO dataset captions), this assumption may not hold. In such cases, the benefits of our projection and fusion mechanism may diminish. 


==> tex/plots.tex <==
% %------------------------------------------------------------------------------
% % hack for CVPR/ICCV style
% \makeatletter
% \@namedef{ver@everyshi.sty}{}
% \makeatother

%------------------------------------------------------------------------------
% main packages
%\PassOptionsToPackage{dvipsnames,svgnames,x11names,table,xcdraw}{xcolor}
\usepackage[dvipsnames,svgnames,x11names,table,xcdraw]{xcolor}
\usepackage{tikz}
\usetikzlibrary{arrows.meta,shapes,calc,matrix,fit,positioning,through,backgrounds,decorations.markings,fadings}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=1.9}
\usepgfplotslibrary{fillbetween}
\usepackage{xstring}
%------------------------------------------------------------------------------
% pgfplots options

\tikzset{every mark/.append style={solid}}
\pgfplotsset{
	grid=both, width=\columnwidth, try min ticks=5,
	every axis/.append style={font=\scriptsize},
	every axis plot/.append style={thick,mark=none,mark size=1.2,tension=0.18},
	legend cell align=left, legend style={fill opacity=0.8},
}

\pgfplotsset{
	dash/.style={mark=o,dashed,opacity=0.7},
	dott/.style={mark=o,dotted,opacity=0.7},
}

==> tex/related.tex <==
\section{Related work}
\label{sec:related}

% \subsection{Composed Image Retrieval}

\textbf{Methods.}
While early methods like TIRG~\cite{tirg}, CIRPLANT~\cite{cirr} and CLIP4CIR~\cite{combiner} rely on supervised training with annotated triplets, recent efforts in zero-shot CIR (ZS-CIR) avoid triplet supervision and fall into three main categories. \emph{Textual-inversion} methods (\eg Pic2Word~\cite{pic2word}, SEARLE~\cite{searle}, ISA~\cite{isa}, LinCIR~\cite{lincir}) map the reference image to a pseudo-text token, which is then composed with the modification text in the language domain and processed by a vision-language model. \emph{Pseudo-triplet} approaches (\eg TransAgg~\cite{transagg}, HyCIR~\cite{hycir}, CompoDiff~\cite{compodiff}, CoVR-2~\cite{covr}, MCL~\cite{mcl}) generate synthetic training data using LLMs~\cite{llava} and image generative models~\cite{stablediffusion}, either from caption-editing strategies or from natural web-based image pairs. \emph{Training-free methods} (\eg \weicom~\cite{pke+24}, FreeDom~\cite{freedom}, CIReVL~\cite{cirevl}, GRB~\cite{grb}, WeiMoCIR~\cite{wu2024training}) leverage off-the-shelf VLMs~\cite{clip, blip, blip2} and LLMs~\cite{llama2} to perform CIR without any additional training by either recasting it as text-based retrieval or fusing visual and textual embeddings directly via weighted sums or geometric interpolations.

\textbf{Datasets.}
%FashionIQ~\cite{fashioniq} is a fashion-focused dataset containing 30,000 triplets and 77,684 images across three disjoint sub-tasks: dress, shirt, and toptee. CIRR~\cite{cirr} is an open-domain composed image retrieval dataset with 21,552 open-domain natural images, and it consists of 36,554 triplets. CIRR is criticized in the literature~\cite{searle} for containing a significant number of false negatives and for allowing many queries to be resolved using text-to-image retrieval alone. CIRCO~\cite{searle} uses the 120,000 images of the COCO 2017 unlabeled dataset~\cite{lmb+14} as distractors, and it consists of 1,020 queries with an average of 4.53 ground-truth targets each. Four domain conversion datasets were introduced in earlier work~\cite{freedom}, where the domain name is used to define the textual queries. ImageNet-R~\cite{imagenet_r} features 30,000 stylized renditions of 200 ImageNet-1K~\cite{dsl+09} classes across four domains: cartoon, origami, sculpture, and toy. MiniDomainNet~\cite{minidomainnet} contains \textasciitilde{}140K images across 126 classes and four domains: clipart, painting, real, and sketch. It is repurposed for retrieval by treating the test split as queries and the rest as the database. NICO++~\cite{nico++} contains 88,866 real-world images across 60 categories and six contexts as domains. For retrieval, 10\% of images are used as queries. LTLL~\cite{leuven} includes 500 images of 25 locations taken over 150 years, divided into ``archive'' and ``today'' domains.
Key benchmarks include FashionIQ~\cite{fashioniq} (77k images, 30k triplets across three fashion sub‐tasks) and CIRR~\cite{cirr} (22k images, 37k triplets), both criticized for label ambiguity, high false‐negative rates, and text‐only shortcuts~\cite{searle, collm}, and recently refined by~\cite{collm}. CIRCO~\cite{searle} (1k queries over 120k COCO‐unlabeled distractors, 4.53 targets/query) extends this paradigm with more diverse negatives. Four additional domain‐conversion datasets-ImageNet‐R~\cite{imagenet_r} (30k stylized images of 200 classes in four style domains), MiniDomainNet~\cite{minidomainnet} (140k images of 126 classes in four domains), NICO++~\cite{nico++} (89k images of 60 categories in six contexts), and LTLL~\cite{leuven} (500 images of 25 locations)-explore class-level retrieval under style or context shifts. Concurrent to our work, ConCon-Chi~\cite{conconchi} introduces an image–caption benchmark for personalized concept–context understanding, designed for text-to-image generation, retrieval, and editing. Their \emph{concepts} correspond to our \emph{instances}, while their \emph{contexts} parallel the modifications expressed by our \emph{text queries}.

% Current CIR benchmarks often suffer from label ambiguity, where modification text lacks clarity, potentially matching multiple target images.

% \subsection{Instance-Level Retrieval}

==> tex/teaser.tex <==
%------------------------------------------------------------
% place teaser between title and abstract
\makeatletter
\apptocmd\@maketitle{{\teaser{}}}{}{}
\makeatother
%------------------------------------------------------------
\newcommand{\teaser}{%
	%\vspace{-28pt}
	\footnotesize
	\centering
	\setlength{\tabcolsep}{4pt}
	\renewcommand{\cellalign}{bc}
        \vspace{-16pt}
	\begin{tabular}{c @{\hspace{6pt}} @{\hspace{6pt}} ccccc}

		% ---------------- first header row ----------------
		& \\
		& \txtbox{in an old\\archival photo} %
		& \txtbox{during sunset} %
		& \txtbox{from an aerial\\viewpoint} %
		& \txtbox{at night,\\with full moon}
            & \txtbox{as a scale model} \\%[18pt]
% 		\cline{2-5}

		%& \texttt{\makecell{in an old\\archival photo}}
		%& \texttt{\makecell{during sunset}}
		%& \texttt{\makecell{from an aerial\\viewpoint}}
		%& \texttt{\makecell{at night,\\with full moon}} \\
            \addlinespace[2pt]
		% ---------------- second row: images -------------------
		\imgbox[.12]{teaser/query_sounio.jpeg} &
		\fig[.12]{teaser/sounio_archival.jpg} &
		\fig[.12]{teaser/sounio_sunset.jpg} &
		\fig[.12]{teaser/sounio_aerial.jpeg} &
		\fig[.12]{teaser/sounio_full_moon.jpg} &
            \fig[.12]{teaser/sounio_scale.jpg} \\

		\textcolor{imagequerycolor}{\makecell{image query}}
		& \multicolumn{5}{c}{\makecell{composed \textcolor{ForestGreen}{positives}}} \\%[2pt]
		%\cline{2-5}

		% -------------- third row: images ---------------------
		\fig[.12]{teaser/temple.jpg} &
		\fig[.12]{teaser/archival.jpg} &
		\fig[.12]{teaser/sunset.jpg} &
		\fig[.12]{teaser/irakleia_aerial.jpg} &
		\fig[.12]{teaser/full_moon.png} &
            \fig[.12]{teaser/scale.jpg} \\

		visual hard \textcolor{gray}{negative} &\multicolumn{5}{c}{textual hard \textcolor{gray}{negatives}} \\%[2pt]
		%\cline{2-5}

		% -------------- fourth row: images ------------------------
		\phantom{} &
		\fig[.12]{teaser/sounio_engraving.png} &
		\fig[.12]{teaser/agrigento_sunset.jpg} &
		\fig[.12]{teaser/lindos_aerial.jpg} &
		\fig[.12]{teaser/acropolis_full_moon.jpg} &
            \fig[.12]{teaser/acropolis_scale.jpg} \\

		&\multicolumn{5}{c}{composed hard \textcolor{gray}{negatives}} \\

		%\cline{2-5}

	\end{tabular}

	\captionof{figure}{We introduce \emph{i}-nstance-level Composed Image Retrieval (\dataset) evaluation dataset. Given an \textcolor{imagequerycolor}{image query} depicting a specific instance (\eg, Temple of Poseidon) along with a modifying \textcolor{textquerycolor}{text query}, the task is to retrieve images showing the same instance altered according to the text (composed \textcolor{ForestGreen}{positives}). Unlike existing datasets~\cite{fashioniq, cirr, searle}, \dataset explicitly ensures the presence of challenging \textcolor{gray}{negative} examples across three distinct dimensions: visual, textual, and composed.}
	%\captionof{figure}{We introduce \emph{i}-nstance-level Composed Image Retrieval (\dataset) evaluation dataset. Given an \textcolor{imagequerycolor}{image query} depicting a specific instance (\eg, Temple of Poseidon) along with a modifying \textcolor{textquerycolor}{text query}, the task is to retrieve images showing the same instance altered according to the description in the text (composed \textcolor{ForestGreen}{positives}). Unlike existing datasets~\cite{fashioniq, cirr, searle}, \dataset explicitly ensures the presence of challenging \emph{negative} examples across three distinct dimensions: identical or visually similar instances without textual modifications (visual hard \textcolor{gray}{negatives}), unrelated images matching fully or partially the textual description (textual hard \textcolor{gray}{negatives}), and similar instances incorrectly modified or partially matching the composed query (composed hard \textcolor{gray}{negatives}).}
	\label{fig:teaser}
	\par\vspace{8pt}
}

==> tex_arxiv/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction accurately summarize our key contributions: the creation of an instance-level composed image retrieval dataset (\dataset) with challenging hard negatives, the proposal of a training-free CIR method (\ours) that leverages existing VLMs, and the demonstration of state-of-the-art performance on \dataset and multiple benchmarks. All claims are supported by detailed methodology and experiments in Sections 3–5, as also in supplementray material.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: We explicitly acknowledge in Sec.~3 (footnote) that our logical‐AND assumption may break down when one modality dominates (e.g., pure style edits or highly entangled image–text pairs like CIRCO). We point readers to additional method and dataset limitations in the supplementary material.  
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper contains no formal theorems or theoretical results requiring proof; it is entirely empirical and algorithmic.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: We give exhaustive details of our dataset construction (including LAION search and retrieve, filtering and annotation protocols) and our method (all pre-processing steps, corpora generation, hyper-parameters $k,\lambda,\alpha$, normalization statistics), and we commit to releasing both the dataset and code with scripts to reproduce every result.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{}
    \item[] Justification: Both \dataset dataset and code will be made publicly available through our project page \url{https://vrg.fel.cvut.cz/icir/}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: The experimental section of both the main paper and supplementary material is exhaustive and detailed. It specifies all the details needed to understand the results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: Our method is training-free, so it does not involve sources of randomness such as weight initialization, optimization, or data shuffling.  
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Technical and implementation details are included in the supplementary material.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: We use only publicly available, license-annotated sources (\eg, LAION-derived URLs and rights-cleared repositories), and we respect licenses and site Terms of Service. All images in \dataset{} were reviewed by trained annotators; inappropriate, copyrighted, or privacy-sensitive content was removed. In categories where people are inherently present (\eg, apparel), we automatically pixelate faces and perform spot checks; no raw PII is released. \dataset{} is an evaluation-only benchmark, distributed under CC-BY-NC-SA with an explicit prohibition on surveillance/biometric or other privacy-invasive uses. We publish a misuse policy, provide a “Report misuse/PII” channel, honor takedown requests, and reserve the right to revoke access for violations. Our method is training-free and does not scrape private data, minimizing environmental and privacy risks. No human-subjects research was conducted (IRB not applicable). Overall, collection, curation, release, and documentation follow the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper explicitly discusses benefits and risks. On the positive side, instance-level composed retrieval can support cultural-heritage search (GLAM), assistive-vision use cases, product provenance, and reproducible evaluation of compositional models. On the negative side, we analyze dual-use pathways—including surveillance/profiling, indirect “object-of-interest” tracking (\eg, via distinctive belongings), fine-tuning our techniques on face/plate corpora, and misuse of crawl scripts—and we describe harms from both correct and incorrect system behavior. However, we exhaustively outline concrete mitigations too.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{}
    \item[] Justification: We release \dataset{} as an \emph{evaluation-only} benchmark under CC-BY-NC-SA with an explicit ban on surveillance/biometric and other privacy-invasive uses; access is governed by a misuse policy with revocation. Images are curated with a privacy-first process: annotators preferentially exclude PII, and in categories where people are intrinsic (\eg, apparel) we retain images but \emph{exhaustively pixelate} visible faces before release; we also filter watermarks, near-duplicates, and low-quality items, followed by manual spot checks. Any search/crawl scripts are released under the same restrictive license with hard-coded keyword blocks and documentation discouraging sensitive-content collection (IRB review recommended for modifications). The project page provides a prominent “Report misuse / PII” channel; we commit to prompt review, content takedown, and access revocation when warranted. We will periodically red-team object-level re-identification risks and update the release if failure modes are found. No identification models or person-level embeddings are released; our method is training-free and not tailored to biometric tasks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: We build on publicly available assets and cite them in the paper and project page. For data, we rely on LAION \emph{metadata} (CC-BY 4.0) and keep each image under its original source license. For models/code, we use public VLMs and toolchains under their original licenses and cite them: CLIP (MIT), OpenCLIP (Apache-2.0), and, for anonymization, InsightFace (MIT). Our own release is evaluation-only under CC-BY-NC-SA and does not alter upstream terms; LICENSE files and attributions are included in our repo.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}
    \item[] Justification: We release \dataset with a comprehensive datasheet detailing collection protocols, licensing, annotation guidelines, dataset statistics, and limitations; our code repository includes installation instructions, example scripts, configuration files for all experiments, and explicit CC-BY-NC-SA license information.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerYes{}
    \item[] Justification: We did not use crowdsourcing; all annotations were performed by salaried institutional staff. The supplemental material includes annotation guidelines/instructions. Annotators received domain and ethics training, and we ran weekly QA spot-checks and inter-annotator-agreement audits. Compensation exceeds the legal minimum (>\,80\% of a first-year PhD stipend with full social-security coverage). No participants were recruited, no demographic attributes were collected, and PII was removed/redacted; thus this work does not constitute human-subjects research, but we nevertheless followed our institution’s ethics policies throughout.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: This work does not constitute human-subjects research: no participants were recruited or interacted with; annotators were salaried staff performing routine labeling; no demographic or behavioral data were collected; and all images were sourced from public datasets with PII removed/pixelated prior to release. Under these conditions, IRB (or equivalent) review is not required per common definitions and institutional policies.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{}
    \item[] Justification: The core method development in this research does not involve LLMs.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> tex_arxiv/method_old.tex <==
\section{Method}
\label{sec:method}


Our approach is a training-free retrieval framework that enhances composite queries in the CLIP embedding space. The core idea is to remove irrelevant or noisy variation from image features and emphasize semantically meaningful directions using lightweight, deterministic transformations. This is done through a set of empirically validated, conceptually simple steps that we consider as a form of \emph{best practices} for zero-shot retrieval. These include modality-specific mean subtraction, projection into a semantic subspace derived from text embeddings, textual contextualization, query expansion, and principled score normalization and fusion.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{fig/cir_methodology.pdf}
    \caption{\emph{Overview of our training-free composed image retrieval \ours method}. Given a query image and text, we apply mean subtraction and semantic projection (guided by corpora $\mathcal{C}+$ and $\mathcal{C}-$) to filter irrelevant dimensions. The text query is contextualized using caption-like prompts. Both modalities are scored against database items with min-based normalization, then fused via a multiplicative “AND” operation regularized by a Harris-like criterion to retrieve jointly relevant results.}
    \label{fig:methodology}
\end{figure}

\subsection{Motivation}

We begin with the assumption that a composite retrieval query consists of two distinct semantic paths—typically, an image and a textual description—each encoding meaningful content. CLIP provides aligned representations across these modalities, enabling retrieval via similarity comparison in a shared embedding space. However, in practice, CLIP embeddings often encode both content and spurious dimensions: visual embeddings are entangled with background, composition, and dataset-specific style; text embeddings reflect lexical biases or corpus-level drift.

Our method assumes that \emph{each modality provides a semantically coherent, complementary path} towards the retrieval goal. This makes the retrieval task analogous to performing a logical “AND” over the two modalities: we seek results that are simultaneously relevant to both the image and the text. This assumption holds well for standard composite tasks (e.g., this image and the concept ``winter”), but may not apply in tasks where one modality dominates (e.g., purely textual transformations) or where the text query is highly entangled with image content (e.g., CIRCO-like datasets). We revisit this in the limitations.




\subsection{Definitions}

We have a dataset of images $I_D$ and image and text queries $I_q$ and $I_t$. 
In this work we rely on corpora to find a proper semantic projection space.
We have the subject-oriented corpus $C_{+}$ and the stylistic-oriented corpus $C_{-}$. Both have textual descriptions and are pre-defined by the user.
We extract the embeddings of all these data using multi-modal feature extractors $\phi_i(\cdot)$ and $\phi_t(\cdot)$, one for each modality, like CLIP.  


Let $I_D$ be the image database and $(I_q, T_q)$ the image and text components of a retrieval query. Features are extracted using pretrained multi-modal encoders $\phi_i(\cdot)$ and $\phi_t(\cdot)$ (e.g., CLIP), mapping images and text into a shared embedding space $\mathbb{R}^d$.
\[
\phi_i(I) \in \mathbb{R}^d, \quad \phi_t(T) \in \mathbb{R}^d.
\]

\textcolor{red}{filby -> its better to define what exactly we want the projection to do before describing it}


To construct a semantic projection space, we use two user-defined textual corpora: 
$\bullet$ $\mathcal{C}_{+}$: a \textit{subject-oriented corpus} capturing content-relevant concepts (e.g., ``building'', ``dog'').
$\bullet$ $\mathcal{C}_{-}$: a \textit{stylistic corpus} capturing distractors such as appearance, lighting, or background style (e.g., ``origami'', ``sunset'').
These corpora guide the projection step: $\mathcal{C}_{+}$ acts as a set of semantic \emph{attractors}, while $\mathcal{C}_{-}$ defines directions to suppress.


\subsection{Mean Subtraction for Bias Removal}

The first step removes modality-specific biases by subtracting mean embeddings, which typically capture low-level regularities that differ between the two modalities. The mean of image CLIP embeddings often reflects “imageness”, while the mean of textual embeddings captures generic “textness”. Removing these helps isolate semantic content from distributional priors.

%Let $\phi(I), \phi(T) \in \mathbb{R}^d$ be image and text embeddings. 
Specifically, we subtract the mean of image embeddings $\mathbf{\mu}_{\text{vis}}$, removing common visual pattern irrelevant to the semantic information,
and the mean of the text corpus $\mathbf{\mu}_{\text{text}}$ (here we use the mean of $\mathcal{C}_{+}$ embeddings), removing common linguistic drift.

While dataset-specific visual means can boost retrieval performance, they assume access to a curated and thematically consistent dataset—an unrealistic assumption in many real-world scenarios. For scalability and generalization, we instead favor using a generic visual mean, estimated from external datasets (e.g., LAION). This allows our method to operate effectively across diverse and unstructured domains without retraining or adaptation.

\subsection{Contextualization of Text Queries}

CLIP is trained primarily on natural language captions and full sentences, rather than isolated category names or sentence parts. As a result, using single-word prompts (e.g., ``sculpture'') or part-sentences (e.g., ``during sunset") may produce such ``partial" representations that are not well-aligned with image embeddings. To address this, we introduce a \emph{contextualization} step that enriches sparse textual queries with compatible noun phrases.

Let $T_q \in \mathbb{R}^d$ be the raw text query (e.g., ``sculpture'') and let $\mathcal{C}_{+}$ be a fixed context vocabulary (e.g., a set of common nouns like ``dog'', ``train'', etc.). For each query, we generate multiple caption-like prompts by combining it with elements from $\mathcal{C}$. We add a random set of nouns before ("dog + during the sunset") and after ("sculpture + dog") the text query. These composed phrases are embedded using CLIP’s text encoder and averaged. 

This operation yields a more robust, subject-aware textual feature that better reflects how CLIP interprets concepts in natural language (e.g., ``[something] during the sunset"). This step is particularly effective when the raw query consists of abstract categories or adjectives (e.g., ``ancient'', ``wooden'', ``patterned'').

\paragraph{Practical Efficiency.} This step requires only one forward pass through CLIP’s text encoder for a fixed set of composed prompts and can be cached per corpus. It adds no inference cost during retrieval.

\subsection{Projection onto Semantic Subspace}

% On the core of this proposed approach, we aim to assist the image query by stripping out any semantically irrelevant information from the image modality. In other words, we want the image embeddings to be projected into a sub-space where we have information only for the ``main character" of the image, the subject. 

The goal of the projection step is to suppress semantically irrelevant information from image features, thereby isolating features related to the image's main subject.


To isolate semantically meaningful directions, we project the centered image features into a lower-dimensional subspace derived from text CLIP embeddings. This projection acts as a filter, suppressing components that do not align with concepts present in the textual domain.

Specifically, we construct the semantic subspace by applying PCA to a corpus of text embeddings $\mathcal{C}_+$. Additionally, we introduce a negative corpus $\mathcal{C}_-$ consisting of distractor concepts (e.g., stylistic terms). From these, we compute their contrastive covariance:

\[
\mathbf{C} = (1 - \alpha) \mathbf{C}_{+} - \alpha \mathbf{C}_{-}, \quad \text{where} \quad \mathbf{C}_{\pm} = \frac{1}{|\mathcal{C}_\pm|} \sum_{x \in \mathcal{C}_\pm} (x - \mathbf{\mu}_{text})(x - \mathbf{\mu}_{text})^\top,
\]

and obtain the top $k$ (< $d$) eigenvectors, forming a projection matrix $\mathbf{P}_r$ that reduces dimensionality from $d$ to $k$. The projected image features are then calculated as 
%\[
$\mathbf{P}_r^\top (\phi(\mathbf{I}) - \mathbf{\mu}_{img}) = \mathbf{P}_r^\top \mathbf{\bar{x}} $.
%\]

This projection captures content-relevant variations and discards common or irrelevant ones. Notably, the text corpus used to compute $\mathbf{P}_r$ need not match the retrieval dataset's domain. Even general corpora (e.g., ImageNet class names) yield performance improvements, because the directions they capture are semantically rich and broadly transferable. By describing the content-relevant part of the image as a linear combination of the basis function of such corpora, we cannot only perform class-based retrieval~\cite{}, but also extend to instance-level retrieval. 

An important implementation aspect can be derived by exploring the similarity score of the image modality. According to our formulation, we can calculate the retrieval similarity between the centered query embedding $\mathbf{\bar{x}}_q$ and the centered embedding of a sample from the dataset $\mathbf{\bar{x}}_i$ by computing the following inner product:
\[
s_i = \langle \mathbf{P}_r^\top \mathbf{\bar{x}}_i,  \mathbf{P}_r^\top \mathbf{\bar{x}}_q \rangle =\mathbf{\bar{x}}_i^\top \mathbf{P}_r\mathbf{P}_r^\top \mathbf{\bar{x}}_q = \mathbf{\bar{x}}_i^\top (\mathbf{P} \mathbf{\bar{x}}_q) ,
\quad \text{where} \quad \mathbf{P} = \mathbf{P}_r \mathbf{P}_r^\top
\]
Note that the projection matrix $\mathbf{P}$ (which does not reduce dimensionality anymore), can be only applied to the query embeddings, avoiding any extra operation on the dataset side.  
\subsection{Query Expansion}

In tasks with high intra-class variation or viewpoint diversity (e.g., instance-level landmark retrieval), it can be beneficial to refine the query representation using the retrieval database. We implement a simple but effective form of \emph{query expansion}.

Given the initial projected query $\mathbf{P}^\top \mathbf{\bar{x}}_q$, we compute its top-$k$ nearest neighbors in the database. These are aggregated into an expanded query via a soft attention-weighted mean:

\[
\mathbf{\tilde{x}}_q = \sum_{i=1}^k w_i \mathbf{\bar{x}}_i, \quad w_i \propto \exp(\beta \cdot \text{sim}(\mathbf{P}^\top \mathbf{\bar{x}}_q, \mathbf{\bar{x}}_i)).
\]

The resulting embedding is then reprojected into the semantic subspace. This step improves robustness by incorporating appearance variation that is semantically consistent with the original query, especially given the fact that the neighboring samples are calculated on the projected space and thus focusing only on the subject and not potential noise.

\subsection{Score Normalization and Fusion}

The final step is to combine similarities from the image and text modalities and rank database items accordingly. Following the aforementioned definitions, we have:
%Let $\hat{\phi}(D)$ be the (projected) embedding of a database item. We compute:

\[
s^{\text{img}}_i = \langle \mathbf{P}^\top \mathbf{\tilde{x}}_q, \mathbf{\bar{x}}_i \rangle, \quad s^{\text{text}}_i = \langle \mathbf{\bar{x}}_t, \mathbf{\bar{x}}_i \rangle.
\]
where $\mathbf{\bar{x}}_t = \phi_c(T_q) - \mathbf{\mu}_{text}$ is the centered contextualized version of the text query $T_q$.

Moreover, zero similarity in one modality could diminish the results, but in a multiplication paradigm this zero "neutral" similarity could better correspond to 1, the neutral element of multiplication.

Following the ``AND'' rationale for combining modalities, the composite similarity for a database item $i$ is computed as:
\[
s_i = s^{\text{img}}_i \cdot s^{\text{text}}_i.
\]
This multiplicative fusion emphasizes candidates that are jointly relevant to both the image and text queries. However, the raw similarity scores $s^{\text{img}}$ and $s^{\text{text}}$ may lie in different numerical ranges due to modality differences, centering, and the image-space projection. This imbalance can lead to one modality dominating the other during fusion.

Additionally, a score of zero in one modality (often the result of mean subtraction or semantic irrelevance) would collapse the product to zero, even if the other modality provides a strong signal. Under this paradigm, it is more appropriate to treat a zero similarity as a ``neutral'' signal—closer in behavior to 1, the multiplicative identity.

\paragraph{Min-Based Normalization.}

To address these issues, we apply a simple normalization strategy that rescales each similarity score based on its empirical lower bound:
\[
\tilde{s} = \frac{s - s_{\min}}{|s_{\min}|}, \quad \text{where } s_{\min} < 0.
\]
This maps $s = s_{\min}$ to 0 and $s = 0$ to 1, treating zero similarity as the neutral value. Such normalization preserves meaningful contrast and ensures that modality scores are better balanced before fusion. 

We apply this function to both $s^{\text{img}}$ and $s^{\text{text}}$ similarities using predefined statistical values for $s^{\text{img}}_{\min}$ and $s^{\text{text}}_{\min}$ that take into account the CLIP backbone, as well as the projection. For more details see suppl. material.

\textcolor{red}{harris can be one sentence}
\paragraph{Fused Similarity with Harris Criterion.}

We can then fuse the normalized scores using a multiplicative operator and a regularizer inspired by the Harris corner detector. The final score is:

\[
\tilde{s}_i = \tilde{s}^{\text{img}}_i \cdot \tilde{s}^{\text{text}}_i - \lambda \cdot (\tilde{s}^{\text{img}}_i + \tilde{s}^{\text{text}}_i)^2.
\]

The first term rewards items that are jointly relevant to both modalities. The second term penalizes cases where only one modality is highly activated, thereby suppressing false positives from unbalanced queries. The scalar $\lambda$ controls the trade-off and is fixed across all experiments.

\subsection{Computational Complexity and Efficiency}

One of the key strengths of our approach lies in its efficiency and simplicity. The entire pipeline is training-free and composed of operations that scale linearly with the dataset size:

\begin{itemize}
    \item \textbf{Centering and projection} are applied once per embedding and require matrix-vector multiplications of $O(dk)$, where $k \ll d$.
    \item \textbf{Similarity computation} is done via matrix multiplication ($O(nk)$ for $n$ database items), which is efficiently handled by existing libraries (e.g., FAISS).
    \item \textbf{Query expansion} adds negligible cost as it only involves top-$k$ retrieval and weighted averaging.
    \item \textbf{No normalization per query or feature is required at test time}. All embeddings are precomputed; query evaluation consists of fast dot products and scalar operations.
\end{itemize}

This makes our method particularly well-suited for large-scale deployments, requiring no adaptation, no fine-tuning, and no backpropagation.

\subsection{Limitations}

Our method assumes that both image and text components of a query provide semantically distinct and complementary information. This allows us to interpret fusion as a logical “AND” operator. However, in tasks where one modality dominates (e.g., text-only edits) or where the text query is highly entangled with image content (e.g., CIRCO dataset captions), this assumption may not hold. In such cases, the benefits of our projection and fusion mechanism may diminish. 

